DT-DDNN: A Physical Layer Security Attack Detector in 5G RF Domain for CAVs

The Synchronization Signal Block (SSB) is a fundamental component of the 5G New Radio (NR) air interface, crucial for the initial access procedure of Connected and Automated Vehicles (CAVs), and serves several key purposes in the network's operation. However, due to the predictable nature of SSB transmission, including the Primary and Secondary Synchronization Signals (PSS and SSS), jamming attacks are critical threats. These attacks, which can be executed without requiring high power or complex equipment, pose substantial risks to the 5G network, particularly as a result of the unencrypted transmission of control signals. Leveraging RF domain knowledge, this work presents a novel deep learning-based technique for detecting jammers in CAV networks. Unlike the existing jamming detection algorithms that mostly rely on network parameters, we introduce a double-threshold deep learning jamming detector by focusing on the SSB. The detection method is focused on RF domain features and improves the robustness of the network without requiring integration with the pre-existing network infrastructure. By integrating a preprocessing block to extract PSS correlation and energy per null resource elements (EPNRE) characteristics, our method distinguishes between normal and jammed received signals with high precision. Additionally, by incorporating of Discrete Wavelet Transform (DWT), the efficacy of training and detection are optimized. A double-threshold double Deep Neural Network (DT-DDNN) is also introduced to the architecture complemented by a deep cascade learning model to increase the sensitivity of the model to variations of signal-to-jamming noise ratio (SJNR). Results show that the proposed method achieves 96.4% detection rate in extra low jamming power, i.e., SJNR between 15 to 30 dB. Further, performance of DT-DDNN is validated by analyzing real 5G signals obtained from a practical testbed.

==> Sections/conclusion.tex <==
\label{conclusion}
This work presents a robust deep-learning-based approach to detect smart and barrage jamming attacks in 5G networks with a particular focus on 5G SSB. By incorporating deep cascade learning and DWT, our DT-DDNN architecture provides remarkable accuracy in classifying a wide range of jamming scenarios, including those characterized by high SJNR values and diverse signal transmission settings. A preprocessing block is integrated to extract PSS correlation and EPNRE characteristics of the received signal which has enhanced the ability of the model to differentiate between the jammed and non-jammed observations. Inclusion of a DWT block in the model, the performance of the training process has enhanced and the training duration is reduced while maintaining the accuracy of the detection. Our results show that DT-DDNN outperforms the single threshold approach and provides more robustness and sensitivity to different jamming scenarios. DT-DDNN demonstrates improved detection probability by 10.4\% and 13.2\% compared to single threshold design and unprocessed IQ sample DNN design respectively. Furthermore, the adaptability of the model has been verified via several experiments with varied channel conditions, delay spread, and jamming techniques. The provided outcomes highlight the effectiveness of the suggested approach which precisely identifies jammer presence in the network with minimal false positive and miss-detection. Additionally, an experimental setup is built to assess the performance of the proposed DT-DDNN model in response to real 5G signals. The experiments conducted on the data collected from the testbed confirm the effectiveness of the system in practical scenarios.
Our ongoing research includes investigation of the potential of unsupervised generative models in jamming detection to improve the performance of the system in the detection of unseen and novel jamming attacks. Furthermore, combining the CFO estimator with the design is expected to transfer the preprocessing load partially to the machine learning block.
Our ongoing research includes investigation of the potential of unsupervised generative models in jamming detection to improve the performance of the system in the detection of unseen and novel jamming attacks. Furthermore, combining the CFO estimator with the design is expected to transfer the preprocessing load partially to the machine learning block.

==> Sections/detector.tex <==
\label{detector}
This section focuses on the proposed jamming detection scheme. The overall block diagram of our detection model is demonstrated in Fig. \ref{fig:block diagram}.
Received signal observations are processed through a data preprocessing module, following which the modified dataset is input into a Deep Learning block for training and jamming detection. The details of each block are provided in the rest of this section.

\graphicspath{{figures/}}
\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth, height=10cm]{figures/block-diagram.png}
    \caption{The block diagram of the proposed detection technique using information from SSB}
    \label{fig:block diagram}
\end{figure*}
% ___________Preprocessing___________
\subsection{Data Preprocessing}
\subsubsection{PSS correlation}
Each transmitted SSB includes a PSS sequence which is a version of one of the three base PSS sequences formulated in (\ref{eq: m-sequences}). Thus, within the correlation signal of the received PSS sequence $y_{pss}(t)$ with one of the m-sequences, we expect to observe a visible peak value.
The correlation of $y_{pss}(t)$ with each m-sequences results in a 1 by 2$N_{FFT}$ signal demonstrated as\footnote{Since there is a specific $x^{ssb}_l(t)$ signal for each $N_{ID}^{(2)}$, the output of the correlator in (\ref{eq:pss corr}) is sub-scripted with $N_{ID}^{(2)}$. },

\begin{equation}\label{eq:pss corr}
\begin{split}
    \boldsymbol{\mathcal{R}_{N_{ID}^{(2)}}}(t)& = \Bigg|\sum_{\tau=0}^{N_{FFT}-1}y_{pss}(\tau)x^{ssb}_l(t-\tau) \big|_{l=0} \Bigg|,\\
\end{split}
\end{equation}

where $|.|$ denotes the absolute value. By analyzing the correlation sequences, the cell ID parameter of the correspondent gNB can be specified. The jammer can distort this cell ID extraction process through jamming signals. 

\subsubsection{DWT}
%\textcolor{red}{Please change the parameter names in Fig. 2,  I changed the correlator output symbol to $\boldsymbol{\mathcal{R}_{N_{ID}^{(2)}}}(t)$, and the output of the DWTs to $\boldsymbol{\mathcal{R}^1_{N_{ID}^{(2)}}}(app)$, and $\boldsymbol{\mathcal{R}^2_{N_{ID}^{(2)}}}(app)$} for the first and second DWT respectively. \\

To remove the redundant information from the correlator output and to magnify the jammer-related features, DWT is employed. This also reduces the dimension of the data set and hence, significantly decreases the training time as described in \ref{Sec: Single Threshold}. As illustrated in Fig. \ref{fig:block diagram}, two-stage DWT is applied to the output of the correlator, $\boldsymbol{\mathcal{R}_{N_{ID}^{(2)}}}(t)$. The approximate output of the first DWT module, $\boldsymbol{\mathcal{R}^1_{N_{ID}^{(2)}}}(app)$, is fed to the second DWT module, generating the final outputs $\Big(\boldsymbol{\mathcal{R}^2_{N_{ID}^{(2)}}}(app) , \, \boldsymbol{\mathcal{R}^2_{N_{ID}^{(2)}}}(det)\Big)$. This process can be mathematically explained as follows:
\begin{equation}\label{eq:DWT2}
\begin{split}
    \big(\boldsymbol{\mathcal{R}^2_{N_{ID}^{(2)}}}(app) , \, \boldsymbol{\mathcal{R}^2_{N_{ID}^{(2)}}}(det)\big)=\\
    & \hspace{-15mm}  \frac{1}{\sqrt{2N_{FFT}}} \sum_m \boldsymbol{\mathcal{R}^1_{N_{ID}^{(2)}}}(app)\psi_{app,det}(t) ,
\end{split}
\end{equation}
\noindent in which $\boldsymbol{\mathcal{R}^1_{N_{ID}^{(2)}}}(app)$ is obtained as,
\begin{equation}\label{eq:DWT}
\begin{split}
   \big(\boldsymbol{\mathcal{R}^1_{N_{ID}^{(2)}}}(app) , \, \boldsymbol{\mathcal{R}^1_{N_{ID}^{(2)}}}(det)\big)= \\
   & \hspace{-15mm} \frac{1}{\sqrt{2N_{FFT}}}\sum_m \boldsymbol{\mathcal{R}_{N_{ID}^{(2)}}}(t)\psi_{app,det}(t).
\end{split}
\end{equation}
where $\boldsymbol{\mathcal{R}_{N_{ID}^{(2)}}}(t)$ is derived as per (\ref{eq:pss corr}).
 Furthermore, $\psi_{app,det}(t)$ is the mother wavelet function chosen as Haar wavelet \footnote{Haar wavelet is a set of rescaled square-shaped functions that collectively form the simplest wavelet family or basis \cite{stankovic2003haar}.} to maintain and magnify the important information from PSS correlation. Haar wavelet is a straightforward choice as it is very effective at identifying abrupt changes in the signal amplitude including PSS peaks \cite{liu2021applications}\cite{tang2018haar}. Thus, it can successfully reduce signal size while maintaining crucial information and keeping the computational load at a desired stage. Fig. \ref{fig:dwt effect} demonstrates the effect of adding two layers of DWT to the PSS correlation dataset. As can be seen in the figure, the length of the correlated signal is decreased by almost 25\%, and the correspondent peak is magnified significantly by 2 times. 
\begin{equation}
    \psi(t)=\begin{cases}
    1,\ \ \ &0\leq t <\frac{1}{2},\\ 
    -1,\ \ \ &\frac{1}{2}\leq t<1\\
    0,\ \ \ &otherwise
\end{cases}
\end{equation}
\vspace{-5mm}
\graphicspath{{figures/}}
\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{figures/dwt.pdf}
    \caption{Applying DWT to the original dataset. The blue line is the signal before DWT and red line demonstrates the effect of DWT on the signal.}
    \label{fig:dwt effect}
\end{figure}

\subsubsection{Energy per Null RE (EPNRE)}
Upon reception of the transmitted signal, it undergoes conversion into the frequency domain through Fourier transform, as depicted in Equation (\ref{eq: fourier of rx}). 
\begin{equation}\label{Eq_fourier of rx}
    Y_{l,k}^{ssb}=\frac{1}{N_{FFT}}\sum_{t=0}^{N_{FFT}-1}y_l^{ssb}(t)e^{-j\frac{2\pi}{N_{FFT}}k t}
\end{equation}
\noindent in which $Y_{l,k}^{ssb}$ represents the Fourier transform of the received signal in $l$-th OFDM symbol and $k$-th subcarrier data point.
In the next step, the SS block is extracted from the frequency domain signal. There are $N_{nre}=113$ numbers of resource elements in the SS block which are intentionally set to zero by gNB as shown in Fig. \ref{fig:ssb}. These resource elements help us collect information about the noise and jamming signal. The energy of these resource elements is calculated as expressed in (\ref{eq:energy}). %\textcolor{red}{please change the formulae in Fig.2, I replace the parenthesis with $\Big|.\Big|$, moreover, since we do not have the variable n defined in the summation, I changed it to k}
\begin{equation}\label{eq:energy}
\begin{split}
    E &=  \frac{1}{N_{nre}}\sum_{k} \Big|{Y_{l,k}^{ssb}\mid_{l=0}} \Big|^2 \\
    k&\in{\{0,55\}}\cup{\{184,240\}}
\end{split}
\end{equation}
Depending on the jammer transmit power and its distance to the UE, the received energy of the jamming signal might be small in some observations. Thus, to adjust the dynamic range of the calculated received energy to be more distinguishable, a log function is applied to the final energy value as,
\begin{equation}\label{eq:log}
    \varepsilon = \log_2(E)
\end{equation}

In the absence of a jammer, the UE is only affected by environmental noise. The energy of this type of interference is significantly small compared to the energy from a jammer. Thus, when the $\varepsilon$ reaches a specific threshold, it can be concluded that a jammer is present in the scenario. %\noteBK{Indeed the impact of $\varepsilon$ may be questioned, so an empirical study could be helpful; not necesarily in this phase but we should be prepared for that.}

% ___________DNN Model___________ 
% DNN model structure
%% optimization problem
%% hyper parameter set table (minibatch,...)
\subsection{DL Block}
\subsubsection{DNN Input}
Observations are designed as a 2-D image including the PSS correlation signals at the output of the second DWT module ($\boldsymbol{\mathcal{R}^2_{N_{ID}^{(2)}}}(app), \, N_{ID}^{(2)}\in\{0,1,2\}$), and energy per null resource elements ($\varepsilon$).
In each observation ($N_{obs}\in\{1,2,...,2\mu_j\}$), the first three rows in the 2-D image include correlated signal, and the last two rows are dedicated to the energy parameter (Fig. \ref{fig:block diagram}). The calculated EPNRE is a scalar value while the size of $\boldsymbol{\mathcal{R}^2_{N_{ID}^{(2)}}}(app)$ is equal to $N_{FFT}/2$. Thus, to maintain the impact of the energy feature and to make it visible to the classifier, the energy is repeated in the last two rows as, \vspace{-3mm}

\begin{equation}\label{eq:repeat E}
    \begin{split}
        \boldsymbol{\mathcal{E}} &= \varepsilon\times{\mathbb{I}}
    \end{split}
\end{equation}
where $\mathbb{I}$ denotes a $(1 \times N_{FFT}/2)$ vector of ones. 
After creating a 2-D image of features, each observation is positioned behind the previous observation thus creating a 3-D tensor (Fig. \ref{fig:block diagram}) as the final dataset ($\boldsymbol{\chi}$).

\begin{equation}\label{eq:final dataset}
    \boldsymbol{\chi}=[\boldsymbol{\mathcal{R}^2_0}^T(app),\boldsymbol{\mathcal{R}^2_1}^T(app),\boldsymbol{\mathcal{R}^2_2}^T(app),\boldsymbol{\mathcal{E}}^T,\boldsymbol{\mathcal{E}}^T]^T
\end{equation}

\subsubsection{Data Augmentation and Class Balancing}
%During the data generation, a noticeable dissimilarity in sample sizes between the two classes has been observed 
The dissimilarity in sample sizes between the two classes, although frequently seen in the process of data collection, causes the class imbalance that must be resolved to maintain the reliability and validity of the produced data. These imbalanced classes can result in biased models and fail to generalize to minority class \cite{johnson2019survey}\cite{buda2018systematic}. This situation causes the CNN model to demonstrate less efficiency and accuracy in classifying the minority observations and decreases the performance of the model in detecting underrepresented received signals. Various techniques, including oversampling the training samples to produce a comparatively balanced dataset \cite{lv2021enhanced}, have been suggested as solutions to this problem. Additionally, research has demonstrated that CNN decisions are more difficult to generalize to minority classes when the data is unbalanced \cite{dablain2023understanding}. However, methods including data augmentation have demonstrated efficacy in enhancing the precision of classification tasks involving unbalanced datasets \cite{rojhani2023model}, \cite{cai2022spectrum}, \cite{gul2023secure}, \cite{li2021influence}, \cite{zheng2021spectrum}. while adversarial machine learning approaches have shown promising solutions in securing wireless systems through augmentation of real data samples \cite{liu2022adversarial}, qualitative and quantitative analyses of various data augmentation techniques are provided in several works, notably in \cite{mumuni2022data}, \cite{shorten2019survey}, \cite{maharana2022review}, \cite{gul.wiseml22}. To overcome the effect of the imbalance classes and use a more robust dataset, circular shift is applied to the minor dataset \cite{zhang2020circular}. Through the circular shift augmentation method, each observation in the minority class is divided into sub-sequences with similar lengths, and each sub-sequence is independently shuffled to create a new sequence which introduces new variations of the collected observations. Traditional techniques (such as rotation, cropping, and flipping) may affect data integrity or eliminate vital information. Circular shift enhances the generalization capabilities of the DNN model by introducing diverse patterns while maintaining most of the original information without significant information loss  \cite{zhang2020circular}, \cite{singh2023systematic},.

\subsubsection{DNN Structure}
The deep learning model used for training is a supervised model, and dataset is paired with the correspondent labels as $(\boldsymbol{\chi}, \boldsymbol{\mathcal{Z}})=\{(\boldsymbol{\chi}^1,\boldsymbol{\mathcal{Z}}^1),(\boldsymbol{\chi}^2,\boldsymbol{\mathcal{Z}}^2),...,(\boldsymbol{\chi}^{\eta},\boldsymbol{\mathcal{Z}}^{\eta})\}$, where $\eta$ is the total number of observations. In this algorithm two classes are represented for the dataset, therefore, $\boldsymbol{\mathcal{Z}}^{\eta}$ represents a binary digit set and can be written using one-hot encoding (\ref{eq: label set}).
\begin{equation}\label{eq: label set}
    \boldsymbol{\mathcal{Z}}^{\eta}=\begin{cases}
        [0\ \ 1]^T\ \ \ \ for\ H_0\\
        [1\ \ 0]^T\ \ \ \ for\ H_1
    \end{cases}
\end{equation}
After normalizing using the softmax layer, the output score of the model for $\eta$-th observation is expressed as follows:
\begin{equation}\label{eq: normalized z}
    \boldsymbol{O}^{\eta}=\begin{cases}
        \zeta_{H_0}(\chi^\eta|\theta)\ \ \ \ for\ H_0\\
        \zeta_{H_1}(\chi^\eta|\theta)\ \ \ \ for\ H_1
    \end{cases}
\end{equation}
\noindent where $\theta$ represents the parameter of the deep learning model, and $\zeta_{H_{i}}(\chi^\eta|\theta)\triangleq P_r\big(\chi^\eta|H_{i},\theta\big), i\in{0,1}$ denotes the jamming scores of the jamming detection problem which satisfies $\zeta_{H_{0}}(\chi^\eta|\theta)+\zeta_{H_{1}}(\chi^\eta|\theta)=1$. Based on the decision rule, two scores are compared and the hypothesis with the higher score becomes the output (\ref{eq: decision}). 
\begin{equation}\label{eq: decision}
    \zeta_{H_{0}}(\chi^\eta|\theta)\underset{H_1}{\overset{H_0}{\gtrless}}\zeta_{H_{1\vee1}}(\chi^\eta|\theta)
\end{equation}

As the features are organized in 2-D images, the deep learning model is designed using 2-D CNN layers. After exploring various architectures and experimenting under different model parameters, the optimal design for the DNN is finalized as demonstrated in Fig. \ref{fig:dnn}. The 3-D tensors including the features of each observation are used as an input to three layers of 2-D CNN with ReLu activation. After each layer of CNN, a batch normalization layer is added to provide faster and more stable training. Two fully connected layers and a softmax layer are used as the last layers of the design. The softmax layer enables the normalization of the output scores. A detailed list of parameters for the DNN model is provided in Table \ref{tab:hyperparameter}.

\begin{table}[htbp]
\caption{Hyperparameter Setting }
\begin{center}
\begin{tabular}{|c|c|}
\hline
Parameter & Value \\
\hline\hline
Mini-Batch Size & 25\\
\hline
Initial Learning Rate & 0.001\\
\hline
MaxEpoch & 20\\
\hline
Validation frequency & 80\\
\hline
CNN-1 & $(2\times5) @ 256$\\
\hline
CNN-2 & $(2\times5) @ 128$\\
\hline
CNN-3 & $(1\times2) @ 128$\\
\hline
FC-1 Output Layer & 128\\
\hline
FC-2 Output Layer & 2\\
\hline
Training Optimization Method & SGDM\\
\hline
Validation Training Rate & 30\% \\
[1ex]
\hline
\end{tabular}  
\end{center}
\label{tab:hyperparameter}
\end{table}

\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=8cm, height=8cm]{figures/dnn-model.png}
    \caption{DNN model.} 
    \label{fig:dnn}
    %\vspace{-2mm}
 \end{figure}

\subsubsection{Offline Training}
% Math explanation
In the classification layer, the main goal is to maximize the probability of detection. Thus, maximizing $\zeta_{H_{0}}(\chi^\eta|\theta)$ in the absent of the jammer and $\zeta_{H_{1}}(\chi^\eta|\theta)$ in the presence of the jammer. To optimize the solution, an objective function can be defined as the Maximum Likelihood (ML) function represented in (\ref{eq: ML}). 

\begin{equation}\label{eq: ML}
    L(\theta)= \prod_{\eta=1}^{N_{obs}} \big(\zeta_{H_{0}}(\chi^\eta|\theta)\big)^{\boldsymbol{\mathcal{Z}}^{\eta}}\big(\zeta_{H_{0}}(\chi^\eta|\theta)\big)^{1-\boldsymbol{\mathcal{Z}}^{\eta}}
\end{equation}

To minimize the loss between the actual and predicted value, a negative log-likelihood function is minimized to adjust the weights during the training as shown below:
\begin{equation}\label{eq: negative LL}
\begin{split}
    \mathcal{H}(\theta)&=-\frac{1}{N_{obs}}\log(l(\theta))\\
    &=-\frac{1}{N_{obs}}\sum_{\eta=1}^{N_{obs}} \boldsymbol{\mathcal{Z}}^{\eta} \log\big(\zeta_{H_{0}}(\chi^\eta|\theta)\big)+\\
    &\ \ \ \ \  \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \ \ \  \ \ \ (1-\boldsymbol{\mathcal{Z}}^{\eta})\log\big(\zeta_{H_{1}}(\chi^\eta|\theta)\big)
\end{split}
\end{equation}
Therefore, the optimization problem can be expressed as (\ref{eq: optimization dnn1}). 
\begin{equation}\label{eq: optimization dnn1}
    \Theta = \arg\min_{\theta}\mathcal{H}(\theta)
\end{equation}
Through stochastic gradient descent (SGD) optimization, the model is trained to provide higher values for $\zeta_{H_{0}}(\chi^\eta|\Theta)$ when $\boldsymbol{\mathcal{Z}}^{\eta}=[1\ \ 0]^T$ or $\zeta_{H_{1}}(\chi^\eta|\Theta)$ when $\boldsymbol{\mathcal{Z}}^{\eta}=[0\ \ 1]^T$. The training is formed through iterative back-propagating processes.


% ___________Double Threshold___________
\subsection{Accuracy Enhancement}
% histogram
% double threshold model \gamma_1, \gamma_2 (D)
\subsubsection{Double Threshold DNN}
The ratio between the two output scores of the detection model can be defined as $\Gamma(\chi^\eta)=\frac{\zeta_{H_1}(\chi^\eta|\Theta)}{\zeta_{H_0}(\chi^\eta|\Theta)}$. This value is compared with a threshold to enable the algorithm to make a detection decision. However, for the scenarios where SJNR value is high, meaning that the jamming signal is weaker compared to the transmitted signal from gNB, the uncertainty at the output of the classifier is high. Thus, the output scores are too close to each other, making it challenging for the classifier to make a decision. In other words, defining one hard decision at the output layer of the classifier reduces the accuracy of the jamming detector in the uncertainty area. To optimize the performance of the detection algorithm, this trade-off between the $P_D$ and $P_{FA}$ should be considered. Therefore, an ambiguity area is defined to reach a better and more accurate decision. Based on this, while the decision is being made out of the ambiguity area, the detector detects the absence or the presence of the jammer with 100\% empirical accuracy, balancing between the requirement for high detection rates against the risk of false alarms. To design such structure, two threshold points ($\gamma^{(1)}_1=\Gamma^{(1)}\big(\boldsymbol{\chi}_s^{\eta_1^*}\big), \gamma^{(1)}_2=\Gamma^{(1)}\big(\boldsymbol{\chi}_s^{\eta_2^*}\big)$) are considered. $\boldsymbol{\chi}_s$ represents sorted observations in descending order, and $\eta_1^*, \eta_2^*$ are observations that fall in the areas that the classification decides with high certainty. These thresholds are obtained as,
\begin{numcases}{}\label{eq: eta1}
        \eta^*_1=\arg\min_{\eta}\big(\zeta^{(1)}_{H_0}(\boldsymbol{\chi}_s^\eta|\Theta)<\zeta^{(1)}_{H_1}(\boldsymbol{\chi}_s^\eta|\Theta)\big)\\
        \label{eq: eta2}
        \eta ^*_2=\arg\max_{\eta}\big(\zeta^{(1)}_{H_0}(\boldsymbol{\chi}_s^\eta|\Theta)>\zeta^{(1)}_{H_1}(\boldsymbol{\chi}_s^\eta|\Theta)\big)
\end{numcases}
While $\Gamma^{(1)}(\chi^\eta)<\gamma^{(1)}_1$ or $\Gamma^{(1)}(\chi^\eta)>\gamma^{(1)}_2$, the detector selects $H_0$ or $H_1$ respectively. In the case that $\gamma^{(1)}_1<\Gamma^{(1)}(\chi^\eta)<\gamma^{(1)}_2$, another DNN is trained specifically for higher SJNR values is activated and observations are fed for more accurate analysis to this DNN. This improves the performance of the jamming detection by minimizing the probability of miss-detection (false negatives(FN)) and false-alarms (false positives(FP)), or equivalently, maximizing true positives (TP) and true negatives (TN). The structure of the DT-DDNN model is represented in Algorithm 1. After data is processed in the data preprocessing block, it is fed into the first DNN with a double threshold design. The first DNN calculates $\zeta^{(1)}_{H_0}(\boldsymbol{\chi}_s^\eta|\Theta)$ and $\zeta^{(1)}_{H_1}(\boldsymbol{\chi}_s^\eta|\Theta)$ which are the weight scores correspondence to this block. These scores are then used at the input of the first threshold and decision block (i.e., Threshold and Decision I). If the scores represent values outside of the uncertainty area, the final decision $Q_1$ is provided as an output. In the case that the score values fall into the uncertainty area, data is sent to the second DNN with a single threshold design for final classification. The second DNN is specifically trained in high SJNR regime to extract more fine-grained features and is expected to yield higher accuracy compared to the first DNN. In the second DNN, the threshold $\gamma^{(2)}$ is used to detect the jammer in harsher conditions (i.e., higher SJNR values). The ratio between the two output scores of the second DNN, $\zeta^{(2)}_{H_1}(\hat{\chi})$ and $\zeta^{(2)}_{H_0}(\hat{\chi})$, is defined as $\Gamma^{(2)}(\chi^\eta)=\frac{\zeta^{(2)}_{H_1}(\hat{\chi})}{\zeta^{(2)}_{H_0}(\hat{\chi})}$. The comparison between the ratio $\Gamma^{(2)}(\chi^\eta)$ and detection threshold $\gamma^{(2)}$ enables a degree of freedom to have a trade-off between $P_D$ and $P_{FA}$. After finding the $\Gamma^{(2)}(\chi^\eta)$ using optimum parameters of $\Theta$ and the $H_0$, empirical $P_{FA}$ can be computed to determine the threshold value. Assume we define the target value for $P_{FA}$ as $\delta_{FA}$ so that $P_{FA} \leq \delta_{FA}$, and we define the total number of observations fallen into $H_0$ hypothesis as $N_{H_0}$. After sorting the observations in descending order ($\chi_s^\eta$), the $\gamma^{(2)}$ threshold can be defined as in (\ref{eq: gamma2}). 
\begin{equation}\label{eq: gamma2}
    \gamma^{(2)}=\Gamma^{(2)}\big(\chi_s^\eta \lfloor \delta_{FA} N_{H_0} \rfloor;\Theta \big)
\end{equation}
The classification is processed based on comparing the ratio of the scores ($\Gamma^{(2)}(\chi^\eta)$) and single threshold value ($\gamma^{(2)}$) in the second DNN. During the online detection, samples are used as input to the DNN block, and after evaluations and passing through the softmax layer, two output scores are presented. The final decision is made in threshold and decision block using $\gamma^{(2)}$ as below:
\begin{equation}\label{eq: final decision}
    \Gamma^{(2)}(\chi_{online})\underset{H_0}{\overset{H_1}{\gtrless}}\gamma^{(2)}
\end{equation}
\noindent in which $\chi_{online}$ represents the online samples. Fig. \ref{fig:dnn2} provides an overall overview of the structure of the double threshold enabled design explained above.

% optimization problem (-10 to 20 dB)

\begin{comment}
\begin{numcases}{}\label{eq: gamma1}
    \gamma^{(1)}_1=\Gamma\big(\boldsymbol{\chi}_s^{\eta_1^*}\big)\\
    \label{eq: gamma2}
    \gamma^{(1)}_2=\Gamma\big(\boldsymbol{\chi}_s^{\eta_2^*}\big)
\end{numcases}
\end{comment}



\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=8.5cm, height=2.5cm]{figures/dnn2.png}
    \caption{Adding another DNN block to improve the accuracy.} 
    \label{fig:dnn2}
    %\vspace{-2mm}
 \end{figure}

\begin{algorithm}
\caption{DT-DDNN - Online Detection}\label{alg:cap}
\begin{algorithmic}[1]
\State Set $\hat{\chi}$ as the current observation
\State Set $\gamma^{(1)}_1=\Gamma\big(\hat{\chi}), \gamma^{(1)}_2=\Gamma\big(\hat{\chi})$
\State Calculate $\zeta^{(1)}_{H_0}(\hat{\chi}), \zeta^{(1)}_{H_1}(\hat{\chi})$
\State Calculate $\Gamma^{(1)}=\frac{\zeta^{(1)}_{H_1}(\hat{\chi})}{\zeta^{(1)}_{H_0}(\hat{\chi})}$

\If{$\Gamma^{(1)}<\gamma^{(1)}_1$}
    \State The classification decides $H_0$
\ElsIf{$\Gamma^{(1)}>\gamma^{(1)}_2$}
    \State The classification decides $H_1$
\ElsIf{$\gamma^{(1)}_1<\Gamma^{(1)}<\gamma^{(1)}_2$}
    \State Activate DNN-2
    \State Calculate $\zeta^{(2)}_{H_0}(\hat{\chi}), \zeta^{(2)}_{H_1}(\hat{\chi})$
    \State Calculate $\Gamma^{(2)}=\frac{\zeta^{(2)}_{H_1}(\hat{\chi})}{\zeta^{(2)}_{H_0}(\hat{\chi})}$
    \If{$\Gamma^{(2)}<\gamma^{(2)}$}
      \State The classification decides $H_0$
    \ElsIf{$\Gamma^{(2)}\geq \gamma^{(2)}$} 
      \State The classification decides $H_1$
    \EndIf  
\EndIf
%\EndWhile
\end{algorithmic}
\end{algorithm}


 \subsubsection{Deep Cascade Learning}
 % to avoid vanishin gradient problem due to low dynamic range of SJNR in our dataset
 %% it accommodates the nonlinear relationship between input and output by not eliminating the linear relationship between the two
 %% efficient training of deep neural networks in a bottom-up fashion using a layered
 %% when sjnr values are close to each other and classifier has troubles classify between two classes so it fine tunes the weights
 Although the convolution network has demonstrated remarkable performance and results \cite{gu2018recent} \cite{mukherjee2020energy}\cite{solanki2022spectrum}\cite{xing2022spectrum}%\cite{krichen2023convolutional}
 , it experiences the vanishing gradient problem while undergoing training \cite{noh2021performance}. This occurs because the weight updates during back-propagation are substantially reduced as the depth of the network increases, meaning that layers closer to input experience a slower learning rate \cite{marquez2018deep},\cite{ali2023scene}.
 %for initial layers due to the low dynamic range of SJNR in our dataset. 
 One solution to overcome this situation is the deep cascade learning algorithm proposed in \cite{marquez2018deep}. Deep cascade learning gradually trains the network from the lowest to higher layers. When the jamming signal is weak and therefore SJNR values are close to each other, the classifier faces trouble classifying between two classes. Deep cascade learning fine-tunes the weights by dividing the network into sub-layers and sequentially trains each layer until all the input layers have been trained. Through this technique, the vanishing gradient problem can be eliminated by compelling each layer of the network to acquire features that are correlated with the output. In other words, it maintains the linear correlation between input and output while accommodating the nonlinear relationship \cite{gautam2021comparative}. Furthermore, it has shown a significant reduction in training time and memory while adjusting the complexity of the network to the given data \cite{marquez2018deep}\cite{wang2021revisiting}\cite{du2019transfer}. The structure of the DNN model using deep cascade learning is shown in Fig. \ref{fig: dcl}. The input layer is connected to the output using two dense layers. The weights for the initial model layer and the output are subsequently obtained via a back-propagation algorithm during the training. After reaching a state of stability, the second layer is trained by connecting to an output layer with a similar structure to the first layer using data created by forward propagating the actual inputs through the fixed initial layer. Through several iterations, every layer goes through this process for learning, and the weights remain constant for the subsequent layer. Adapting this approach helps increase the robustness of the second DNN and preserve the back-propagated gradient while having hidden layers. 
\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figures/cascade.png}
    \caption{Deep Cascade Learning model} 
    \label{fig: dcl}
    %\vspace{-2mm}
 \end{figure}

==> Sections/introduction.tex <==
%-------------------What is 5G SSB----------------------------------
The evolution in transformative technologies such as Connected and Automated Vehicles (CAVs), the Internet of Things (IoT), and Edge Computing, necessitates the development of next-generation wireless networks to guarantee the Quality of Service (QoS) for communication processes \cite{hamidi20215g}. Given the impact of security attacks on QoS, various defense strategies are proposed to provide detection mechanisms and countermeasures to reduce the impact of these attacks \cite{khan2019survey}\cite{zhang2019towards}\cite{park2021comprehensive}\cite{amini24}. Among these, machine learning-based defense strategies including decentralized and centralized are rising due to their performance in increasing the robustness of the wireless networks \cite{zhang2024federated}.
Moreover, proper operation of critical elements of the network, such as synchronization signal block (SSB), is required to ensure the integrity and security of the communication.
% cite WWRF work
SSB is an essential component in 5G wireless communication systems, as it enables device synchronization with the network and access to the services that are available \cite{tuninato2023comprehensive}. The SSB functions as a reference signal that provides the establishment and maintenance of connections between mobile devices and the base station (gNB). Assisting user equipment (UE), including smartphones and other devices, in synchronizing with the 5G network is the main function of the SSB. 
Effective communication requires synchronization, which guarantees that the UE and the base station operate at the same time and frequency. 
It is crucial that 5G SSBs are robust and resilient to a variety of channel conditions in order to guarantee synchronization that is reliable despite the complexity of the environment. In addition, 5G enables the configuration of SSBs to be more adaptable to various deployment scenarios and facilitates more effective network management.


SSB is transmitted based on predetermined frequency and timing resources in 5G networks \cite{3gpp.38.211}. Due to this predictability, an attacker can target these established locations. By identifying the subcarrier spacing and getting synchronized with the cell in the time domain, an attacker is able to extract the cell identity and as a result, locates and targets PSS or SSS which prevents UE from receiving critical signals required for synchronization \cite{flores2023implementation}, \cite{pirayesh2022jamming}. 
By detecting PSS and SSS, and learning about the PCI, the adversary can execute a jamming attack on PBCH \cite{lichtman20185g}, \cite{wang2023detecting}, \cite{pirayesh2022jamming}. Jamming attacks targeting PBCH in SSB, unable UEs to access necessary information and new connections to cells. Authors in \cite{arjoune2020smart} suggested using localization-based detection techniques as a solution, however, these techniques are not efficient in a mobile jammer scenario.
Another reason behind the vulnerability of SSB is the lack of encryption through initial access. Unlike user data which is encrypted to ensure confidentiality in 5G networks, control signals such as PSS and SSS are transmitted without encryption \cite{wang2023detecting}. Thus, SSB can potentially be jammed by anyone without the requirement of deciphering or authentication. 
Furthermore, an attacker which performs jamming attack on SSB does not require to consume high energy to successfully disrupt the communication \cite{ludant2021sigunder}. Utilizing less jamming power enables the jammer to minimize its impact on the monitoring and detection systems as most of the detection systems rely on identifying anomalous high-energy patterns. On the other hand, it helps the attacker to perform the attack with simple and inexpensive equipment.
Traditional jamming detection methods rely on the received signal intensity, or the performance of the network \cite{arjoune2020real}. The signal level detection methods are incapable of maintaining the detection accuracy in high signal-to-jamming and noise ratio (SJNR) scenarios, and are mostly efficient in constant jamming cases \cite{ornek2022efficient}, \cite{arjoune2020smart}. The detection techniques based on the network metrics such as packet delivery ratio (PDR) or bit error rate (BER) may be unsuccessful when facing advanced jammers utilizing selective or intelligent techniques which may not have a significant impact on the error rate or performance metrics.

%-------------------SSB Jamming Detection---------------------------
% Other possible references:
% SigUnder: a Stealthy 5G Low Power Attack and Defenses, Norbert Ludant Guevara Noubir
% Adversarial Machine Learning for 5G Communications Security, Yalin E. Sagduyu, Tugba Erpek, and Yi Shi
% Towardsimprovedsatellitetelecommandlinkavailability, Nele Noels Ignacio AguilarSánchez
% 5G NR Jamming, Spoofing, and Sniffing: Threat Assessment and Mitigation, Marc Lichtman Raghunandan Rao, Vuk Marojevic, Jeffrey Reed Roger Piqueras Jover
% 5G device-to-device communication security and multipath routing solutions, Aslihan Celik Jessica Tetzner  Koushik Sinha John Matta
% Research on synchronous coherent jamming technology of 5G mobile phone signal,, Haonan Li, Chen Lu, Hongyue Qian, Jinlong Song, Huijun Yang
% Practical Jamming of a Commercial 5G Radio System at 3.6 GHz, Agnius Birutis Anders Mykkeltveit

%Possible solutions: techniques like beamforming to create narrow, focused beams for SSB transmission, implementing interference detection and avoidance strategies, and network-level security measures to detect and respond to jamming attacks.
%-------------------------Contribution------------------------------
% contribution:
% Jamming detection at RF domain (no need to be a network entity) through a deep learning approach (1)
% Focused on SSB to make the algorithm capable to detect both smart and barrage jammer (1)
% Performed preprocessing to extract energy per null subcarrier and correlation features of PSS to increase the detection accuracy (1)
% Performed DWT to magnify the extracted features and to lower the training time (1)
This research presents a jamming detection technique for 5G networks based on a deep learning approach operating solely in the RF domain which eliminates the need for the jamming detector to be an entity of the network. 
A key discriminator that sets our work apart from existing jamming detection algorithms is its focus on the analysis of 5G SSB using the design of a double threshold double DNN model (DT-DDNN) to enable the system to detect both smart and barrage jammers effectively.
This expands the algorithm's applicability and impact by covering a wider range of jamming scenarios. To enhance the precision of the detection algorithm and reduce its time and energy consumption, a preprocessing block is integrated into the design in which correlation and EPNRE characteristics of the PSS are extracted. This step provides a more precise discrimination between normal and jammed receive signals. As the deep learning algorithms require advanced computational resources, we incorporate the Discrete Wavelet Transform (DWT) into our design. The DWT magnifies the features that were extracted during the preprocessing phase, and provides a more detailed representation of the signal attributes. This not only improves the performance of the detection model but also optimizes the training procedure. A significant enhancement to our architecture is the integration of double threshold DNN which has been used to improve precision in the scenarios indicated by higher SJNR values in which the detector faces challenges to make a final decision. The additional DNN is supported by a deep cascade learning model to increase the sensitivity of the design in a high SJNR regime. Therefore, the main contributions of this study are summarized as follows. 
\begin{itemize}
    \item  Utilize over-the-air 5G signal features without the need for higher layer KPIs such as Block Error Rate (BLER), Bad Packet Ratio (BPR), throughput, and other metrics in higher layers of 5G protocol stack. This enables the jamming detection module to be implemented independently in 5G networks,.i.e., the proposed method does not need to be implemented on 5G network entities such as gNB, UE, or 5GC.
    \item Exploit salient features in the SSB that are relevant to jamming signal through preprocessing of the received 5G waveform. Particularly, PSS correlation, DWT, and energy per null subcarriers in SSB are employed. Furthermore, Log transformation is applied to adjust the dynamic range of the extracted energy so that the jamming signal can be better distinguished from environmental noise.
    \item Implement a double-threshold deep learning structure to improve the detection performance in a high SJNR regime and optimize their thresholds. In particular, a double deep learning structure is proposed in which the first DNN uses two thresholds at its output to best determine any uncertainties in the detection process. Exploiting deep cascaded structure, the second DNN decides on the observations with high uncertainty in which the UE experiences very low jamming power. %SJNR between 15 to 30 dB. 
\end{itemize}

%--------------------------Structure--------------------------------

The two thresholds at the output of the first DNN are optimized in a way that 100\% empirical detection rate for the two classes is achieved, and the threshold for the second DNN is chosen empirically based on the target false alarm probability.
Using the proposed techniques enables DT-DDNN to attain a 96.4\% detection rate in low jamming power conditions when SJNR is between 15 dB to 30 dB. The performance improvement is significant when compared to 86.0\% detection rate of the single threshold DNN approach and 83.2\% detection rate of the unprocessed IQ sample DNN method. Furthermore, a testbed is developed for experimental evaluation of the proposed approach which validates the performance of the system in real-world applications.

The rest of this work is organized as follows: Section \ref{relatedwork} discusses the existing works in jamming detection in 5G. Section \ref{sysModel} provides a brief introduction to the 5G SSB and formulates the problem. Section \ref{detector} includes detailed information on the jamming detector design and each component of the architecture. Section \ref{results} presents the results of the detection technique. Finally, conclusions are provided in section \ref{conclusion}.



==> Sections/relatedwork.tex <==
\label{relatedwork}
%----------------Jamming Detection techniques-----------------------
% intro for related works

The primary aim of physical layer security (PLS) is to fulfill the security demands of wireless networks by leveraging the unique characteristics of the physical layer \cite{solaija2022towards}. There has been significant research dedicated to developing techniques for detecting attacks that specifically target the physical layer of wireless communication systems.
In the context of the vulnerabilities associated with 5G Non-Orthogonal Multiple Access (NOMA), \cite{zhang2020physical} discusses challenges that arise when a near-end user (NU) engages in eavesdropping activities. To address this, modifications to the serial interference cancellation (SIC) process through cooperative jamming have been suggested. These modifications aim to devise optimal power allocation strategies tailored to various situations, enhancing the secrecy rates without compromising the data throughput of legitimate users, ensuring it remains within acceptable limits.

% eavesdropping, analytical (optimization problem(inputs: power allocation, constraints: channel gains, total power, SNR threshold, noise power), NOMA
\cite{zhang2020physical} discusses the challenges of 5G Non-Orthogonal Multiple Access (NOMA) while a near-end user (NU) performs an eavesdropping attack. The authors proposed modifying the order of serial interference cancellation (SIC) using cooperative jamming. Optimal power allocation strategies are designed for different scenarios to improve secrecy rates while maintaining the data rate of authorized users within the specific threshold.
% MIMO-NOMA
Authors in \cite{nandan2021beamforming} analyze how the reusability of resources compromises the physical layer security in multiple-input multiple-output NOMA (MIMO-NOMA) scenario in cognitive radio network (CRN). Thus, a transmit-zero-forcing beamforming (ZFBF) method is proposed alongside signal alignment in an environment while primary and secondary users share cells. Furthermore, the eigen beamforming method is used to maximize the signal-to-information-leakage-plus-noise ratio (SLNR) and therefore improve the physical layer security. 
% mmWave NOMA, 
AN innovative minimal angle-difference user pairing scheme is provided in \cite{huang2020physical} to mitigate the impact of eavesdroppers in the millimeter wave (mmWave) NOMA network. This work also presents and assesses two secrecy beamforming models, NMRT and CMRT, which increase the secrecy performance by taking advantage of the spatial correlation between the user and eavesdropper.
% UOWC
The efficacy of physical layer security of the integration of reconfigurable intelligent surface (RIS) and Radio Frequency-Underwater Optical Wireless Communication (UOWC) in a scenario including an eavesdropper is investigated in \cite{hossain2022physical}. 
% mmWave vehicular
\cite{eltayeb2017enhancing} increases the secrecy rate of mmWave vehicular communication in response to eavesdropping attacks by using a multiantenna transmission technique and a robust beamforming model. The beamforming vectors are optimized to guarantee the QoS for authorized users and maximize the secrecy rate at the same time.
% write a sentence to related PLS to jamming
% 5G Het-Net, jamming, federated learning
Authors in \cite{sharma2022mitigating} present a novel anti-jamming technique based on federated deep reinforcement learning (DRL) which is based on a joint beamforming and power allocation optimization problem. By using the Markov decision process (MDP), the optimization problem is transformed into a multi-agent reinforcement learning (MARL) problem. The main purpose of the anti-jamming method is to improve the achievable rate of femtocell users (FUs) during a jamming attack targeting 5G Heterogeneous Networks (Het-Nets). 
% 5G UAV
\cite{viana2023deep} focuses on attack identification in air-to-ground communication links using deep attention recognition (DAtR) which detects security attacks using a small deep network embedded in legitimate unmanned aerial vehicles (UAVs). The system employs two metrics of received signal strength indicator (RSSI) and signal to interference plus noise ratio (SINR) to identify attacks in different scenarios such as non-line-of-sight (NLoS), line-of-sight (LoS), or a combination of both.
% Smart Jammer, statistical(based on blank REs), 5G and beyond
In \cite{chiarello2021jamming} a jamming detection and defense strategy is proposed by implementing pseudo-random blanking of resource elements within OFDM symbols based on statistical hypothesis testing. The work is focused on smart jammers which maximize their impacts by reducing spectral efficiency and BLER values, and minimize their detection probability. Through the detection algorithm, certain subcarriers are left blank across OFDM symbols in a pseudo-random fashion. Adopting a pseudo-random algorithm that determines the blanking pattern makes the system unpredictable and increases its robustness to jamming. The suggested approach incorporates the downlink data transmission system of 5G without necessitating adjustments to the current infrastructure. 
% tone and chirp jammer, threshold-based (based on EVM), 5G
\cite{ornek2022efficient} and \cite{ornek2023securing} present a novel approach that employs the sensitivity of Error Vector Magnitude (EVM) to detect the presence of tone and chirp jammers when the EVM value reaches a predetermined threshold. Besides the high sensitivity and minimal complexity, this approach offers spectral information about the jammer and affected frequency bands.
% different types of jammer, ML with network parameters, 5G
\cite{jere2023bayesian} describes an adaptable, multidimensional strategy for detecting and classifying jamming attacks, considering power levels and frequency band variations. The detection technique is based on supervised learning and receives metrics such as channel quality indicator (CQI), bit rates, packet rates, power headroom, and power headroom. The dataset is generated using a 5G NR non-standalone (NSA) testbed from cross-layer key performance indicator (KPI) data. By combining instantaneous discriminative models along with sequential time series-based models, adaptability is obtained. The use of Reservoir Computing (RC) helps to achieve high accuracy and low false alarm rates while following the latency limits of real-time scenarios and requiring minimal computational and memory resources.
% (constant, random, deceptive, reactive) jammer, XGBOOST-Ensemble learning (using network traffic), 5G
% deceptive jamming: mimics the signal of legit BS
The primary focus of \cite{kouassi2023application} is the utilization of ensemble learning and the XGBOOST-ensemble learning combination as a machine learning-based jamming detection in C-RAN. Authors use the WSN-DS database to assess the performance of various machine learning algorithms. The WSN-DS database includes 374,661 samples as chosen features that encapsulate the behavioral patterns of network traffic under normal and jammed conditions. Data preprocessing is performed to set up the dataset for analysis by separating the independent and dependent variables. The feature extraction process is carried out using the XGBOOST algorithm which emphasizes important patterns within the data. Model training is then developed based on cross-validation with various algorithms to identify the most effective model for detection. The model is finally tested and validated using an independent dataset.
% barrage jammer, Hoeffding decision tree (received signal), 5G
\cite{arjoune2020real} emphasizes the need for real-time detection and mitigation techniques. 
Hence, the authors make a contribution by introducing a technique for real-time detection of jamming attacks, utilizing the Hoeffding decision tree. This machine learning methodology facilitates real-time processing and addresses limitations encountered in conventional decision tree models. The jamming node in the simulation uses numerous antennas to simulate a smart jammer and a comprehensive dataset under congestion and normal conditions is created to feed to the Hoeffding algorithm.
% (constant, random, deceptive, reactive) jammer, ML-intrusion detection (DL with kernelized SVM)(energy consumption, is CH, ADV CH send, ADV SCH send, data sent to BS(number of packets), Distance CH to BS, Data received, ADV CH receives, Join REQ receive, Time), 5G C-RAN
\cite{hachimi2020multi} presents a multi-stage machine learning-based intrusion detection system (ML-IDS) specifically designed for 5G Cloud Radio Access Network (C-RAN) which is designed to detect constant, random, deceptive, and reactive jammers. A Multilayer Perceptron (MLP), a deep learning algorithm, and a Kernelized Support Vector Machine (KSCM) compose the proposed ML-IDS. The MLP is implemented as the main classifier, and in situations where it produces a false negative, the KSVM functions as a supplementary verification mechanism to enhance the precision of jamming attack detection. The ML-IDS is incorporated into the Base-Band Unit (BBU) pool, an essential element of the C-RAN responsible for monitoring spectrum distribution and user information. This enables the ML-IDS to efficiently manage traffic between base stations.
% various types of jammers, supervised ML(downlink/uplink bitrate, downlink/uplink packet rate, downlink/uplink retransmission rate, PUSCH SNR, CQI, power headroom, energy per resource element, uplink path loss, downlink/uplink MCS, and the average turbo decoder rate) unsupervised (waveform), 5G
The integration of supervised and unsupervised learning methods for jamming detection is introduced in \cite{wang2022anonymous}. Known jamming attacks are detected using a supervised learning model while an unsupervised anomaly detection method using auto-encoders is applied for unknown jamming types. To enhance the accuracy of the detection algorithm, address the computational complexity, and causality analysis of KPI degradation, the Bayesian Network Model (BNM) is integrated into the design. The learning-based model is executed based on network parameters such as bitrate, packet rate, retransmission rate, and CQI.
\cite{wang2023detecting} concentrates on intelligent PBCH jamming (PBCH-IJ) attack in 5G NR which disrupts the MIB decoding by applying a sniffing attack to extract PCI information. Based on the observations, authors concluded that the PBCH-IJ has a substantial effect on the principal direction in low mobility scenarios. Thus, the introduced counteract is based on the Principal Direction of PBCH Dominant Space (PDPDS) and is executed at user side. To identify anomalies that can detect the jamming attack, sparse principal component analysis (SPCA) is used in the design along with an adaptive detection threshold.
% This work is on Wifi
The study in \cite{feng2018machine} implements a machine learning-based detection technique using NS-3 simulator for constant, random, and reactive jammers. Received signal strength, carrier sense time, noise, and PDR are used as jamming detection metrics. The detection method is tested based on three different learning algorithms K nearest neighbor (KNN), decision tree, and random forest with the highest accuracy of 81\%.
This work distinguishes itself from the aforementioned research by focusing on smart SSB jamming detection in the RF domain using signal features of 5G network. The detection technique is a machine learning-based model using two DNN blocks one with a single threshold and the second one with double threshold characteristics to be able to detect the existence of the jammer in high SJNR conditions. To further enhance the performance of the DNN model deep cascade learning approach is adapted by the second DNN block. A summary of the current literature is provided in Table \ref{table:detection-compare}.

\begin{table*}[htbp]
    \caption{Overview of physical layer attack detection techniques in literature and this work }
    \label{table:detection-compare}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    Ref. & Technical Approach / Network Model & Feature or Parameter & Attack Type & Real data test \\
    \hline 
        \hline
    \cite{zhang2020physical} & Analytical (optimal power allocation)/NOMA & Transmit Power & NU Eavesdropper & \ding{55}\\
    \hline
    \cite{nandan2021beamforming} & Analytical(ZFBF)/CRN &  Beamforming Vectors & Eavesdropper & \ding{55}\\
    \hline
    \cite{huang2020physical} & Analytical (SOP\tablefootnote{secrecy outage probability})/mmWave NOMA & Transmit Power & Eavesdropper & \ding{55}\\ 
    \hline
    \cite{hossain2022physical} & Analytical (average secrecy capacity, SOP) & RIS element phases & Eavesdropper & \ding{55}\\
    \hline
    \cite{eltayeb2017enhancing} & Analytical (optimal beamforming vector)/ mmWave V2V & CSI\tablefootnote{channel state information}, Transmit Power& Eavesdropper& \ding{55}\\
    \hline
    \cite{sharma2022mitigating} & ML(DRL)/5G Het-Nets &channel, beamforming vectors & intermittent, constant, adaptive, reactive& \ding{55}\\
    \hline
    \cite{viana2023deep} & ML(CNN, LSTM)/5G UAV&SINR, RSSI & jamming & \ding{55}\\
    \hline
    \cite{wang2023detecting} & statistical(SPCA) /5G &PBCH data & PBCH Jamming & \ding{55} \\
\hline
    \cite{arjoune2020real} & ML(Hoeffding Decision Tree)/5G& Received Signal & Barrage Jammer&\ding{55} \\
       \hline
    \cite{ornek2022efficient}\cite{ornek2023securing}& Statistical (EVM)/5G & EVM & Tone, Chirp Jammer& \ding{55}\\
    \hline
    \cite{chiarello2021jamming} & Statistical (GLRT)/5G & NA & Smart Jammer & \ding{55} \\
   
    \hline
    \cite{jere2023bayesian}& ML(Supervised Learning)/5G & Cross-layer KPI & Various Jammer Types & \checkmark \\
    \hline
    \cite{kouassi2023application} & ML(Ensemble Learning)/5G & Network Traffic & Constant,Random,Deceptive,Reactive & \ding{55}\\
     \hline
    \cite{hachimi2020multi} & ML(DL with kernelized SVM)/5G C-RAN &  Network Traffic & constant,random,deceptive,reactive & \ding{55}\\
    \hline
    \cite{wang2022anonymous} & ML(Supervised, Unsupervised Learning)/5G& Network Metrics & WiFi Interference, controlled jamming& \checkmark\\
    \hline
    \cite{feng2018machine} &  ML(KNN, Decision tree, Random Forest)/WiFi& Packet delivery rate, RSS & Constant, Random, Reactive& \ding{55}\\
    \hline
     \cite{viana2023deep} &  ML(KNN, Decision tree, Random Forest)/WiFi& Packet delivery rate, RSS & Constant, Random, Reactive& \ding{55}\\
    \hline
    This work & ML(DT-DDNN) / 5G RF-Domain & PSS Corr, EPNRE & Smart SSB \& Barrage Jamemr & \checkmark\\
    \hline
    \end{tabular}
\end{table*}

\begin{comment}
\begin{table*}[h!]
\caption{Overview of jamming attack detection techniques in literature \noteBK{Broken references}}
\label{table:detection-compare}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c|c|}
\cline{2-9}
                                                                                                                                              & \multicolumn{2}{c|}{\textbf{Network Type}} & \multicolumn{1}{c|}{\textbf{Layer}} & \multicolumn{1} {c|}{\textbf{Technical Approach}} & \multicolumn{1} {c|}{\textbf{Input Features}} \\ \cline{2-9} 
                                                                                                                                              & 5G     & Other    & Proactive    & Reactive      & Function-specific    & Smart-hybrid   & Anti-jamming   &  Parameters  \\ \hline
\multicolumn{1}{|c|}{\cite{wood2003jam}}                                                                                                      &                       &   \checkmark     &           &            &      \checkmark &                &       &     SNR, failure rate, region           \\ \hline
\multicolumn{1}{|c|}{\cite{aziz2015resilience}}                                                                                               &                     &   \checkmark    &   &            &            &      \checkmark          &  \checkmark  &    cell utility  \\ \hline
\multicolumn{1}{|c|}{\cite{varga2022jamming}}                                                                                                          & \checkmark           &                &            &            &  \checkmark    &                &   &     spectrum, data rate          \\ \hline
\multicolumn{1}{|c|}{\cite{ornek2022efficient}}                                                                                              &         \checkmark        &       &            &    &            &        \checkmark        &     &      SJR, EVM, RB, PDR, throughput\\ \hline
\multicolumn{1}{|c|}{\cite{cheng2017time}}                                    &           &     \checkmark            &     \checkmark       &   \checkmark   &            &                &  &        throughput, delay, PDR       \\ \hline
\multicolumn{1}{|c|}{\cite{hachimi2020multi}}                                                                                         &        \checkmark             &       &            &  \checkmark &    &                &   &       energy consumption, accuracy, true/false positive        \\ \hline
\multicolumn{1}{|c|}{\cite{sharma2022mitigating}}                                                                                               &          \checkmark           &        &              & \checkmark  &            &                & \checkmark  &       data rate, throughput, energy efficiency        \\ \hline
\multicolumn{1}{|c|}{\cite{karagiannis2018jamming}}                                                                                               &                     & \checkmark      &    \checkmark         &            & \checkmark   &       \checkmark        &            &   SINR, RSSI, PDR    \\ \hline
\multicolumn{1}{|c|}{\cite{wang2022anonymous}}                                                                        &         \checkmark           &        &   &            &      \checkmark      &                 &  &        accuracy, precision, false/true positive      \\ \hline
\multicolumn{1}{|c|}{\cite{thamilarasu2006cross}}                                                                                                         &                     & \checkmark      &             &             &    \checkmark  &                 &   &   throughput, delay   \\ \hline
\multicolumn{1}{|c|}{\cite{arjoune2020novel}}                                                                                                &        \checkmark              &      &  &            &            &         \checkmark      &   &      detection, false alarm, accuracy         \\ \hline
\multicolumn{1}{|c|}{\cite{nguyen2014real}}                                                                                                  &                     &   \checkmark    &            &      \checkmark      &   &                &            & \acrshort{PRR}, UDP bandwidth,SIR     \\ \hline
\multicolumn{1}{|c|}{\cite{bhattarai2015simulation}}                                                                                                &                    &   \checkmark     &  &            &    \checkmark        &               &   &       throughput, delay, PDR        \\ \hline
\end{tabular}%
}
\end{table*}
\end{comment}

==> Sections/results.tex <==
\label{results}
In this section, dataset generation and the performance of the proposed deep jamming detection architecture in offline training and online testing are evaluated and discussed thoroughly.
\subsection{Simulation results}
%__________Data Generation_________________
\subsubsection{Data generation}
% generate waveform in 4 ofdm symbols including SS block, including random data
% CDL channel
% applying gnb power
%The 5G transmitter, generates a 5G waveform including 4 OFDM symbols. The transmitter is capable of sending signals using four different types of modulation including QPSK, 16QAM, 64QAM, and 256QAM.
% different types of jammer (AWGN, BPSK, QAM)
To collect the received signal recordings, a synthetic 5G dataset is generated from the scenarios with and without jammer under different conditions. The generated dataset is then processed by data preprocessing block and fed into the detection model. A detailed description of the dataset generation environment is provided as follows.

The transmitter produces 5G waveform including four OFDM symbols containing the SS block. It is capable of transmitting the signal using four different types of modulation including QPSK, 16QAM, 64QAM, 256QAM. The signal is then passed through CDL-D channel model and is received by the UE. UE and gNB are positioned in different locations, and the UE is connected to the base stations with different cell IDs. Different locations for the UE results in different path loss experiences. The simulation environment is equipped with free-space path loss model to demonstrate the effect of different UE positions in the scenario as,
\begin{equation}\label{eq:fspl}
    L_{fs}(dB) = 20\log \left(\frac{\lambda^2}{4\pi^2d^2}\right)
\end{equation}
\noindent where $\lambda$ and $d$ signify the wavelength and the distance between gNB and UE, respectively.
The received signal for each observation is recorded in time domain and the number of observations is $\mu$. The same process is performed to record the received signal in the presence of the jammer with different SJNR values and jamming powers. The number of observations in this scenario is denoted as $\mu_j$. The jammer used for the training is designed using AWGN. Other types of jammers such as the jammer which can transmit modulated BPSK, and 8QAM signals are used for testing. The dataset parameters used for the dataset generation are extracted from \cite{3gpp.38.901}, \cite{han2021hybrid} and listed in Table \ref{tab: sim param}. 
\begin{table}[htbp]
\caption{Dataset Parameters}
\begin{center}
\begin{tabular}{|c|c|}
\hline
Parameter & Value \\
\hline\hline
SJNR & -10 to 30 dB, step size: 1 dB \\ \hline
Distance & 10 to 500 m, step size: 20 dB \\ \hline
%Dataset Size $N_{obs}$ & 18600 \\ \hline
Input Size & $5 \times 1024$ \\ \hline
$N_{FFT}$ & 2048\\ \hline
Delay Spread & 30 ns\\ \hline
Subcarrier Spacing (SCS) & 30 kHz\\ \hline
Sample Rate\tablefootnote{The sample rate equals to $SCS\times N_{FFT}$ which equals $61.44 $ Msps} &  61.44 Msps \\ \hline
Antenna Noise Temperature & 290 K\\ \hline
Cyclic Prefix & Normal \\ \hline
Number of Resource Blocks & 106 \\ \hline
Channel Model & CDL-D \\ \hline
gNB Power & 30 dB \\ \hline
Modulation Scheme & QPSK, 16QAM, 64QAM, 256QAM\\ \hline
\end{tabular}  
\end{center}
\label{tab: sim param}
\end{table}
%_______________DNN1_______________________
% training curve  
% ROC (10 dB - 20 dB SJNR)

\subsubsection{Performance under the Single Threshold DNN} \label{Sec: Single Threshold}
The training performance of the first single threshold DNN is presented in Fig. \ref{fig: st-train}. In this figure, the upper graph plots the accuracy of the model which stabilizes around 94.93\% by jumping quickly into the convergence region in the early stages of the training process. The integration of DWT into the design results in more precision and less training time of 144 minutes, while before adding DWT the training time was around 41 hours. The below graph presents the loss plot which demonstrates a sharp drop during the early stages, eventually reaching a state of stability around 0.01. This signifies a decrease in the prediction error as the training proceeds. It can be concluded that the model is capable of classifying the unobserved data without falling into overfitting. 

\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figures/training2.png}
    \caption{Offline training-- single threshold DNN model } 
    \label{fig: st-train}
    %\vspace{-2mm}
 \end{figure}

Fig. \ref{fig: st-conf} presents the confusion matrix for jamming detection with a single threshold DNN design while the SJNR is spanning from -10.5 to 30 dB. The figure demonstrates the performance of the detection algorithm in which true positive (TP) and true negative (TN) correspond to non-jammed and jammed classes respectively. Based on this matrix, the algorithm classified 5322 observations as TP with the rate of 88.0\%, and 5201 cases as TN with the rate of 86.0\%. 12.0\% of the jammed cases were falsely classified as non-jammed scenarios and 14.0\% of the non-jammed observations were erroneously classified as jammed cases. This demonstrates the ability of the model to accurately differentiate between jammed and non-jammed signals. However, it also introduces the potential for further improvement to decrease the misclassification cases particularly to reduce the FN observations. In the jamming detection scenario, reducing FN is more important than FP, as failure to identify a jammer leads to security risks and communication disruption \cite{greco2021jamming}. 

\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=6.5cm, height=6cm]{figures/dnn1-conf.png}
    \caption{Confusion matrix of single threshold DNN-- SJNR from -10.5 to 30 dB} 
    \label{fig: st-conf}
    %\vspace{-2mm}
 \end{figure}

 % DNN1 tests
 % Channel, delay spread
 After training and testing the model, a different test dataset is implemented consisting of signals transmitted over CDL-C and CDL-A channel models with $600ns$ delay spread. The purpose of this test is to show the generalization of the proposed model to various 5G network settings. The confusion matrix in Fig. \ref{fig: channel-conf} demonstrates the robustness of the design to the disparities of the network by correctly detecting 97.3\% of the non-jammed cases and 94.1\% of jammed cases. Furthermore, recall and precision can be obtained as 0.97 and 0.94 respectively. Hence, the model demonstrates minimal misclassification which shows its ability to detect the attack despite increased complexity. This test highlights the potential of the detection model in a real-world 5G network while maintaining performance and accuracy in a more complex test environment.
\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=6.5cm, height=6cm]{figures/channel-conf.png}
    \caption{Confusion matrix of single threshold DNN under test-- The test dataset consists of signals that have been transmitted through CDL-C and CDL-A channel models with a delay spread of $600ns$, the SJNR value is from 0 to 20 dB.} 
    \label{fig: channel-conf}
    %\vspace{-2mm}
 \end{figure}
 
% jamming type 8QAM
Besides testing under different network settings, a second test dataset compromised by a jammer transmitting with 8QAM signal modulation is created to test the effectiveness of the detector model to different types of jamming signals. Based on the confusion matrix of this test which is provided in Fig. \ref{fig: 8qam-conf}, despite using AWGN as the jamming signal in the training process, it demonstrates acceptable flexibility by accurately classifying 97\% of non-jammed cases and 100\% of jammed observations. These results show the robustness of the design against novel jamming techniques which signifies a transfer of learning from one jamming mode to another. However, no percentage of jammed cases were incorrectly classified, which corresponds to zero probability of miss-detection (FP=0). These results demonstrate the ability of the model to stay generalized to various types of jamming without requiring retraining.
\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=6.5cm, height=6cm]{figures/8qam-conf.png}
    \caption{Confusion matrix of single threshold DNN under test-- a test dataset influenced by a jammer using 8QAM modulation.} 
    \label{fig: 8qam-conf}
    %\vspace{-2mm}
 \end{figure}
%_______________DNN2_______________________
% training
% confusion matrix
% ROC/ total
% compare with DNN1
\subsubsection{DT-DDNN Performance}
Fig. \ref{fig: SJNR} demonstrates the relationship between the number of missed class observations and the SJNR in dB. During these experiments, the received power of gNB is fixed to focus solely on the effect of the jammer. It can be observed that as the SJNR increases, there is a significant rise in the number of missed detections. This trend is related to the reduction in the strength of the received jamming signal compared to the power received from the gNB as SJNR increases. As a result, the effect of the jammer on model features is decreased and the received signal pattern is similar to the cases without the jammer, which contributes to a rise in classification error. The observed situation highlights a significant challenge in the jamming detection model as it is more difficult for the detector to distinguish between the jammed and legitimate signals. Thus, in a high SJNR regime, the deep learning model incorrectly classifies jammed signals as normal. One solution to resolve this issue is adding a double-threshold DNN model to the design. The primary objective of this change is to augment the sensitivity of the jamming detection model, particularly in conditions characterized by high SJNR. By employing a double threshold approach, the detection model is capable of conducting a more comprehensive analysis of the signal, distinguishing low-power jamming attacks from regular signal fluctuations which enhances the precision of the model.
\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=6.5cm, height=6cm]{figures/SJNR.png}
    \caption{SJNR vs miss-classed observations} 
    \label{fig: SJNR}
    %\vspace{-2mm}
 \end{figure}
%
\begin{comment}
\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figures/training2.png}
    \caption{Training of double threshold DNN design integrated with cascade learning model.} 
    \label{fig: dt-train}
    %\vspace{-2mm}
 \end{figure}
\end{comment}
%

The confusion matrix of the DT-DDNN design which includes a double DNN architecture to improve the sensitivity of the jamming detector is presented in Fig. \ref{fig: dt-conf}. While the first DNN uses a double-threshold concept to increase the sensitivity, the second DNN includes a deep cascade learning model to enhance the ability of the system to accurately classify complex observations and decrease the probability of miss-detection to 9.0\%. The model accurately classifies 91.0\% of non-jammed cases and 96.4\% of jammed observations, which shows almost 3\% and 10.4\% rise in the accuracy compared to the single threshold architecture. These results represent an advancement in the ability to detect and provide countermeasures for jamming attacks in real-world scenarios of the 5G network. 

\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=6.5cm, height=6cm]{figures/dt-conf.png}
    \caption{Confusion matrix for the DT-DDNN with SJNR ranging from -10.5 to 30 dB.} 
    \label{fig: dt-conf}
    %\vspace{-2mm}
 \end{figure}
% another DNN is also trained with raw IQ samples taken from 5G waveform, IQ-DNN. The optimum configuration achieved with 4 layers of CNN with batch and relue following each layer. 

Comparative analysis of three DNN designs for jamming detection in a 5G network is provided by the ROC curves in Fig. \ref{fig: dt-roc}. The green dotted curve corresponds to a DNN trained on raw IQ samples taken from 5G waveform with no preprocessing block in the design. The optimum configuration was achieved with 4 layers of CNN with batch and ReLu following each layer. The single threshold DNN design, illustrated by the blue dashed curve, is correspondence to the single threshold DNN design that uses a single DNN to classify jammed cases. In contrast, the red solid curve represents the DT-DDNN design which uses a double DNN system to improve the sensitivity of the detection algorithm. The primary DNN block detects jamming by applying a double threshold decision-making method, and the secondary DNN handles observations that fall into the ambiguous area that the first DNN has found difficulties in classifying. By integrating a deep cascade learning model into the second DNN, the objective is to further enhance the classification performance. Based on the ROC curves, it is evident that the DT-DDNN provides a higher probability of detection ($P_D$) in comparison to the majority of false alarm probabilities ($P_{FA}$). This indicates a greater proportion of true positive and a reduced potential of miss-detection of legit signals as jamming. This suggests that the second design with DT-DDNN architecture offers a more robust jamming detection system under challenging detection cases.

\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{figures/DT-ROC.pdf}
    \caption{ROC curves comparing the DNN trained with unprocessed IQ samples and two proposed jamming detection designs. }
    \label{fig: dt-roc}
    %\vspace{-2mm}
 \end{figure}



\subsection{Experimental Validation}



% Experimental setup Description
The experimental evaluation is conducted within the FR1 5G NR n71 band operating within the downlink frequency range of 617-652 MHz and bandwidth of 35 MHz \cite{3gpp.38.104}. During the initial tests, it is concluded that this spectrum is shared between Telus (with carrier frequency of $f_c=632\ MHz$) and Rogers (with carrier frequency of $f_c=622\ MHz$). Data acquisition is performed using ThinkRF spectrum analyzer RTSA R5500 (shown in Fig. \ref{fig: equip}) and two different types of antennas. The location of the test and therefore distance from the gNB is variable during the sampling. The experimental setup is configured with the sample rate of 15.625 MHz, the carrier frequency of $f_c=632\ MHz$, and the intermediate frequency bandwidth (IFBW) of 10\ MHZ. Sampling is conducted in various environments, including indoor (behind the windows and under the desk) and outdoor (Line-of-Sight (LOS) and Non-Line-of-Sight (NLOS)) scenarios and collected samples are stored in CSV format using PyRF4 API. 

\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=7cm, height=6cm]{figures/equipments.jpg}
    \caption{Experimental setup to collect real over-the-air dataset. The testbed includes \emph{thinkRF} RTSA R5500 spectrum analyzer, two types of antennas, and a PC.}
    \label{fig: equip}
    %\vspace{-2mm}
 \end{figure}

% Synchronization with gNB and blind search
To extract precise information of SSB, it is critical to perform time offset (TO) and carrier frequency offset (CFO) estimations. This is due to the lack of knowledge on the exact center frequency, which necessitates the application of a blind search. To accurately calculate the TO and CFO, we utilize the PSS correlation characteristics along with the cyclic prefix from CP-OFDM 5G waveform to fine-tune with gNB signal.
The optimization problem for estimating CFO is formulated as, \vspace{-3mm}
\begin{equation}\label{eq: optimization CFO}
\begin{split}
      \hat{f}_{CFO} &= \arg\max_{f_i} \Bigg[\sum_{\tau} y(\tau)e^{j2\pi \frac{f_i}{f_s}\tau}x^{ssb}_l(t-\tau)  \big|_{l=0} \Bigg],
\end{split}
\end{equation}
For obtaining time offset to the SSB, Schmidl \& Cox approach \cite{Schmidl1997} is adopted which exploits the cyclic prefix in 5G waveform. Hence, the following optimization problem is solved numerically.\vspace{-3mm}

\begin{equation}\label{eq: optimization TO}
\begin{split}
      \hat{t}_{off} &= \arg\max_{t} \, M(t)=\frac{|P(t)|^2}{R(t)^2} ,
\end{split}
\end{equation}
in which $P(t)$ and $R(t)$ are as,

\begin{equation}\label{eq: TO-P}
\begin{split}
      P(t)=\sum_{m=0}^{L-1} y^*(t+m)y(t+m+L)  ,
\end{split}
\end{equation}
and \vspace{-3mm}

\begin{equation}\label{eq: TO-R}
\begin{split}
      R(t)=\sum_{m=0}^{L-1}|y(t+m+L)|^2 
\end{split}
\end{equation}
respectively.
Following the extraction of SSB, the correlation signals and EPNRE values are calculated. Fig. \ref{fig: exp-pss} demonstrates OFDM symbols of SSB versus the subcarrier indices for one of the observations selected as an example. In this figure, black cross markers represent the PSS symbols that are used to calculate PSS correlation, and red dots correspond to null subcarriers from which EPNRE is calculated.
The features of collected samples, including 6000 observations, are then transferred into a 3D tensor and fed into the DT-DDNN model. The threshold parameters of the DT-DDNN which defines the sensitivity of the model are updated based on environmental noise power.

% Extract energy and PSS
\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{figures/exp-pss.pdf}
    \caption{OFDM symbols of the extracted SSB based on subcarrier indices.}
    \label{fig: exp-pss}
    %\vspace{-2mm}
 \end{figure}

% results
The confusion matrix in Fig. \ref{fig: exp-conf} provides an evaluation of the performance of DT-DDNN model using data obtained from the practical testbed. Based on these results, the model accurately classifies 93.6\% of non-jammed cases and 94.1\% of jammed observations. 213 observations of jammed signals are classified as non-jammed cases with a miss-detection rate of 6.4\% and 217 cases of non-jammed observation are classified as jammed observations with false-alarm probability of 5.9\%. These results validate the practical applicability and efficacy of DT-DDNN model by showing the ability of the proposed model to accurately distinguish between jammed and non-jammed 5G signals in experimental configuration. 

\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=6.5cm, height=6cm]{figures/exp-conf.png}
    \caption{Confusion matrix of the performance of DT-DDNN in response to data obtained from the experimental setup.} 
    \label{fig: exp-conf}
    %\vspace{-2mm}
 \end{figure}

==> Sections/system-model.tex <==
\label{sysModel}
% Received SSB = y
%------------------------Background--------------------------------
\subsection{Background}
The SSB is usually transmitted within the 5G radio frame using 4 OFDM symbols \cite{kopacz2021effective} and includes two synchronization signals: the primary synchronization signal (PSS) and secondary synchronization signal (SSS) \cite{lin2018ss}. The SSB comprises information necessary for the UE to establish synchronization with the cell, such as the physical cell identity (PCI) of the cell, and additional information provided by physical broadcast channel (PBCH) and physical downlink shared channel (PDSCH)\cite{lin2018ss}. 
PSS and SSS use the same time slots as the PBCH. PBCH symbols are concentrated in two or four slots, which gives the appearance of a low-duty cycle, particularly at higher subcarrier spacing. The Master Information BLock (MIB), containing critical data transported by the PBCH, comprises parameters that are vital for the UE to establish a connection with a cell.
When a UE powers on or enters a new cell's coverage area, it uses this information to discover the available SSBs. Scanning the predefined SSB locations within the radio frame, the UE executes an SSB discovery procedure to accomplish this. The UE is capable of decoding the information carried by an SSB, including the PCI, once it has been detected.

%------------------------System model Intro-------------------------------------
\subsection{Problem formulation}
%The focus of the rest of the work is on detecting the jamming attack using information from SSB. (D)
% Formulate jamming detection using SSB
% Explain SSB technically
%% Which symbol and slot SSB is in the frame structure (D)
%% Explain about SSB bursts (D)
%% Mention the exact location of the first SSB burst (cite 3GPP) (D)
%% Mention the place of the PSS and SSS in the SSB (1st symbol and 3rd symbol (D)
This section provides an introduction to SSB, as the focus of our detection algorithm is on analyzing information derived from this block. The rest of this section presents a detailed explanation of the 5G system model, along with the formulation of the jamming detection problem. The notations used in this paper are defined in Table \ref{tab:symbols}.

\begin{table}[htbp]
\caption{Description of Notaions } \vspace{-5mm}
\label{tab:symbols}
\begin{center}
\begin{tabular}{ |c|c|c| }
\hline
Symbol & Description & Equation \\
\hline \hline
$\Phi_{N_{ID}}$ & PSS base sequences & \ref{eq: m-sequences}, \ref{eq: tx symbol 0} \\ \hline
$X_{l,k}^{ssb}$ & Transmitted SSB in frequency domain & \ref{eq: tx symbol 0}, \ref{eq: ifft} \\ \hline
$x_l^{ssb}(t)$ & Transmitted SSB in time domain & \ref{eq: ifft}, \ref{eq:rx ssb}, \ref{eq:pss corr}, \ref{eq:hypothesis}, \ref{eq:hypothesis2} \\ \hline
$y_l^{ssb}(t)$ & Received SSB in time domain& \ref{eq:rx ssb}, \ref{eq: rx pss}, \ref{eq:hypothesis}, \ref{eq:hypothesis2}, \ref{eq: fourier of rx}\\ \hline
\multirow{2}{4em}{$y_{pss}(t)$} & Extracted PSS sequence from the received & \ref{eq: rx pss}, \ref{eq:pss corr}\\ 
& signal in time domain & \\ 
\hline
$Y_{l,k}^{ssb}$ & Received SSB in frequency domain& \ref{eq: fourier of rx}, \ref{eq:energy}\\ \hline
\multirow{3}{4em}{$\boldsymbol{\mathcal{R}_{N_{ID}^{(2)}}}(t)$} & Correlation of extracted PSS sequence & \ref{eq:pss corr}, \ref{eq:DWT}\\ 
&from the received signal & \\
& and three m-sequences &\\
\hline
$\boldsymbol{\mathcal{R}^i_{N_{ID}^{(2)}}}$ & Output of $i^{th}$ DWT stage& \ref{eq:DWT}, \ref{eq:DWT2}, \ref{eq:final dataset}\\ \hline
\multirow{3}{4em}{$E, \epsilon, \boldsymbol{\mathcal{E}}$} & Energy per null resource elements, & \ref{eq:energy}, \ref{eq:log}, \ref{eq:repeat E}, \ref{eq:final dataset}\\ 
&log transform of energy, vectorization& \\
& of log transform of energy, respectively& \\
\hline
\multirow{2}{4em}{\ \ \ \ $\boldsymbol{\chi}^i$} & 3-D tensor of $i^{th}$ observation & \ref{eq:final dataset}, \ref{eq: normalized z}, \ref{eq: decision},\\ 
& & \ref{eq: ML}, \ref{eq: negative LL}\\
\hline
$\boldsymbol{\mathcal{Z}}^i$ & Corresponding label for $i^{th}$ observation & \ref{eq: label set}, \ref{eq: ML}, \ref{eq: negative LL}\\ \hline
\multirow{2}{4em}{\ \ \ $\zeta_{H_{i}}$} & Score of the jamming detection algorithm& \ref{eq: normalized z}, \ref{eq: decision}, \ref{eq: ML},\\ 
&  for $i^{th}$ class &\ref{eq: negative LL}, \ref{eq: eta1}, \ref{eq: eta2}\\
\hline
$\gamma$ & DNN model threshold & \ref{eq: gamma2}, \ref{eq: final decision}\\
\hline
\end{tabular}
\end{center}
\end{table}

In the first step of gaining access to a gNB, UE requires information called System Information Block 1 (SIB1) which depends on the decoding of Master Information Block (MIB) \cite{chen2020design}. This procedure is achievable only through the detection of SSB. One or more SSBs are transmitted through an SS burst periodically based on a pre-determined periodicity at a five-millisecond window \cite{3gpp.38.213}. Each SSB contains cell ID information which is calculated by $N_{ID}^{Cell}=3\times N_{ID}^{(1)}+N_{ID}^{(2)}$. Where $N_{ID}^{(1)}\in\{0,1,...,335\}$ represents group ID and $N_{ID}^{(2)}\in\{0,1,2\}$ is related to sector ID \cite{3gpp.38.211}. Sector ID is provided by PSS to help reach a coarse time and frequency synchronization. A 5G frame includes numerous slots, each being divided into a specific number of symbols which depends on the subcarrier spacing and numerology. SSB is transmitted through four OFDM symbols in the time domain and spans over $k_{ssb}=240$ subcarriers in the frequency domain (Fig. \ref{fig:ssb}). 127 subcarriers in the first symbol are dedicated to PSS, and there are 113 unused subcarriers below and above PSS which are set to '$0$'. PSS follows on of the three base $k_{pss}$-symbols m-sequences $\Phi_{N_{ID}^{(2)}}(k)$ in frequency domain. Each m-sequence is a circular shift version of the other two and their cross-correlation value is equal to zero \cite{you2020efficient}. The three base m-sequences are demonstrated in (\ref{eq: m-sequences}).

\begin{equation} \label{eq: m-sequences}
    \begin{split}
        \Phi_{N_{ID}^{(2)},k}&=1-2s(m)\\
        m=(k+43\times N^{(2)}_{ID})&mod \, k_{pss},0\leq k<k_{pss}
    \end{split}
\end{equation}

\noindent where $\Phi_{N_{ID}^{(2)},k}$ demonstrates the PSS symbol at subcarrier $k$, and $k_{pss}$ is the length of the PSS sequence in the frequency domain. Furthermore, $s(m)$ represents the m-sequences which are given as,
\begin{equation}\label{eq: sequence}
\begin{split}
    s(i+7)=(s(i+4)+s(i)&) \ mod \, 2\\
        [s(6) \ s(5) \ s(4) \ s(3) \ s(2) \ s(1) \ s(0)] &= [1 \   1 \ 1 \ 0 \ 1 \ 1 \ 0]
\end{split}
\end{equation} 

\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=.8\linewidth]{figures/5GNRgrid.png}
    \caption{5G Signal Synchronization Block (SSB).}
    \label{fig:ssb}
    %\vspace{-2mm}
 \end{figure}

% 5G Network Model-------------------------------------------------
Consider a gNB generating a waveform $X^{ssb}_{l,k}$ in frequency domain containing the SSB, where $l\in\{0,1,2,3\}$ denotes the OFDM symbol in 5G resource grid and $k\in\{0,1,...,k_{ssb}-1\}$ represents the subcarrier data point. The transmitted SSB includes the PSS sequence in the first OFDM symbol as defined in (\ref{eq: tx symbol 0}).
\begin{equation}\label{eq: tx symbol 0}
    X_{l,k}^{ssb}\big |_{l=0}=\begin{cases}
        \Phi_{N_{ID}^{(2)},k},\ k\in \{56, 57,...,182\}\\
        0,\ \ \ \ \ \ \ \ \ \ \ otherwise
    \end{cases}
\end{equation}
The signal is subjected to modulation and after applying IFFT, the time domain signal ($x^{ssb}_l(t)$\footnote{t here indicates the time index for a discrete-time signal.}) is formed as,  

\begin{equation}\label{eq: ifft}
\begin{split}
    x^{ssb}_l(t)=\frac{1}{k_{ssb}}&\sum_{k=0}^{k_{ssb}-1}X_{l,k}^{ssb}e^{j\frac{2\pi}{k_{ssb}}tk}\\
    l&\in\{0,1,2,3\}
\end{split}
\end{equation}

During the transmission, the transmitted signal experiences the impact of channel model and thermal noise, and it is degraded by the path loss attenuation. Therefore, the received SSB ($y_{l,k}^{ssb}(t)$) having been subjected to the impact of thermal noise ($\sigma_{th}$) and channel model ($h(t)$) is represented in (\ref{eq:rx ssb}) where $N_{FFT}$ represents the number of FFT points.

\begin{equation}\label{eq:rx ssb}
    y^{ssb}_l(t) = \sum_{\tau=0}^{N_{FFT}-1} x^{ssb}_l(\tau) h(t-\tau) + \sigma_{th}
\end{equation}

As the received PSS sequence is transmitted through the first OFDM symbol ($l=0$), it can be extracted by taking the first $N_{FFT}$ samples of the time domain signal as,

\begin{equation}\label{eq: rx pss}
\begin{split}
    y_{pss}(t) &= y_{l}^{ssb}(t)\big|_{l=0}, \\
    t\in\{&0,...,N_{FFT}-1\}
\end{split}
\end{equation}

In the scenario where a jamming signal ($x_j(t)$) is introduced, the received signal becomes susceptible to the impact of the jammer. Detection of the jamming signal can be represented as a binary hypothesis framework (\ref{eq:hypothesis}),(\ref{eq:hypothesis2}), where we have a null hypothesis denoted as $H_0$ and an alternative hypothesis, $H_1$, corresponding to the presence of the jamming signal.

\begin{numcases}{}\label{eq:hypothesis}
    H_0 : & $y^{ssb}_l(t) = \sum_{\tau} x^{ssb}(\tau) h(t-\tau) + \sigma_{th} $ \\ \label{eq:hypothesis2}
    H_1 : & $y^{ssb}_l(t) = \sum_{\tau} x^{ssb}(\tau) h(t-\tau) + \sigma_{th} + x_j[t]$
\end{numcases}
% path loss: d^-v
 Any detection method comes with two main performance metrics which are false-alarm ($P_{fa}$) and detection probabilities ($P_{d}$), or equivalently, false positive (FP) and false negative (FN), respectively.


\begin{comment}
%------------------------------------------------------------------
\section{Proposed DNN-based jammer detection}
This section focuses on the proposed jamming detection scheme. The overall block diagram of our detection model is demonstrated in Fig. \ref{fig:block diagram}.
First, a 5G dataset is generated from the scenarios with and without jammer under different conditions. The generated dataset is then processed using a data pre-processing block. Finally, the processed dataset is fed into a Deep Learning block for training. The details of each block are provided in the rest of this section.

\graphicspath{{figures/}}
\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth, height=10cm]{figures/block-diagram.png}
    \caption{The block diagram of the proposed detection technique using information from SSB}
    \label{fig:block diagram}
\end{figure*}

% ___________Data Generation___________
\subsection{Data generation}
% generate waveform in 4 ofdm symbols including SS block, including random data
% CDL channel
% applying gnb power
%The 5G transmitter, generates a 5G waveform including 4 OFDM symbols. The transmitter is capable of sending signals using four different types of modulation including QPSK, 16QAM, 64QAM, and 256QAM.
% different types of jammer (AWGN, BPSK, QAM)

The transmitter produces 5G waveform including four OFDM symbols containing the SS block. It is capable of transmitting the signal using four different types of modulation including QPSK, 16QAM, 64QAM, 256QAM. The signal is then passed through CDL-D channel model and is received by the UE. UE is positioned in different locations from gNB and it is connected to the base stations with different cell IDs. Different location for the UE results in different path loss experience. The simulation environment is equipped with free-space path loss model to demonstrate the effect of different UE positions in the scenario \ref{eq:fspl}.
\begin{equation}\label{eq:fspl}
    L_{fs}(dB) = 20\log \left(\frac{\lambda^2}{4\pi^2d^2}\right)
\end{equation}
\noindent where $\lambda$ and $d$ signify the wavelength and the distance between gNB and UE, respectively.
The received signal for each observation is recorded in time domain and the number of observations is $\mu$. The same process is performed to record the received signal in the presence of jammer with different SJNR values and jamming powers. The number of observations in this scenario is denoted as $\mu_j$. The jammer used for the training is designed using AWGN. Other types of jammer such as the jammer which can transmit modulated BPSK, and 8QAM signals is used for testing. The dataset parameters used for the dataset generation are listed in Table \ref{tab: sim param}. 

\begin{table}[htbp]
\caption{Dataset Parameter Set Table}
\begin{center}
\begin{tabular}{|c|c|}
\hline
Parameter & Value \\
\hline\hline
Dataset Size $N_{obs}$ & \\
Input Size & \\
$N_{FFT}$ & 2048\\
delay spread & 30 ns\\
Channel Model & CDL-D \\
Modulation Scheme & QPSK, 16QAM, 64QAM, 256QAM\\
[1ex]
\hline
\end{tabular}  
\end{center}
\label{tab: sim param}
\end{table}


% ___________Preprocessing___________
\subsection{Data Preprocessing}
\subsubsection{PSS correlation}
Each transmitted SSB includes a PSS sequence which is a version of one of the three base PSS sequences formulated in \ref{eq: m-sequences}. Thus, by looking at the correlation signal of the received PSS sequence $y_{pss}(t)$ with one of the m-sequences, we expect to observe a visible peak value.
The correlation of $y_{pss}(t)$ with three m-sequences results in a matrix including three 1 by 2$N_{FFT}$ signals demonstrated in Eq.\ref{eq:pss corr}. By analyzing the correlation sequences, the cell ID parameter of the correspondent gNB can be specifies. The jammer can distort this cell ID extraction process by transmitting jamming signal. 

\begin{equation}\label{eq:pss corr}
\begin{split}
    \boldsymbol{R_{pci}}(t)& = \Big|\sum_{\tau=0}^{N_{FFT}-1}y_{pss}(\tau)\phi_{N_{ID}^{(2)}}(t-\tau)\Big|,\\
    pci & \in \{0,1,2\},\\
    \boldsymbol{R}&\in \mathbb{R}^{1\times2N_{FFT}}
\end{split}
\end{equation}

\subsubsection{DWT}
To reduce the training time and the length of data while preserving the important information in the correlated signal, we applied double Discrete Wavelet Transform to the PSS correlation signals. 

\begin{equation}\label{eq:DWT}
\begin{split}
    \boldsymbol{\mathcal{DW}_{R_{pci}}}(app,det)=\frac{1}{\sqrt{2N_{FFT}}}\sum_m \boldsymbol{R_{pci}}(t)\psi_{app,det}(t),\\
    \boldsymbol{\mathcal{R}}_{pci}(app,det)=\frac{1}{\sqrt{2N_{FFT}}}\sum_m \boldsymbol{\mathcal{DW}_{R_{pci}}}(app)\psi_{app,det}(t)
\end{split}
\end{equation}
\noindent in which $\boldsymbol{\mathcal{DW}_{R_{pci}}}(app,det)$ denotes the first layer of DWT and $\boldsymbol{\mathcal{R}}_{pci}(app,det)$ represents the second layer of DWT while $pci\in \{0,1,2\}$. $\psi_{app,det}(t)$ is correspondence to Haar wavelet to maintain and magnify the important information from PSS correlation. Fig. \ref{fig:dwt effect} demonstrates the effect of adding two layers of DWT to the PSS correlation dataset. As can be seen in the figure, the length of the correlated signal is decreased by almost 25\%, and the correspondent peak is magnified significantly by 2 times. 

\begin{equation}
    \psi(t)=\begin{cases}
    1,\ \ \ &0\leq t <\frac{1}{2},\\ 
    -1,\ \ \ &\frac{1}{2}\leq t<1\\
    0,\ \ \ &otherwise
\end{cases}
\end{equation}

\graphicspath{{figures/}}
\begin{figure}[htp]
    \centering
    \includegraphics[width=6.5cm, height=5cm]{figures/dwt.png}
    \caption{Applying DWT to the original dataset. The blue line is the signal before DWT and red line demonstrates the effect of DWT on the signal.}
    \label{fig:dwt effect}
\end{figure}

\subsubsection{Energy per Null RE (EPNRE)}
After receiving the transmitted signal, the signal is converted into the frequency domain using Fourier transform \ref{eq: fourier of rx}. 
\begin{equation}\label{eq: fourier of rx}
    Y_{l,k}^{ssb}=\frac{1}{N_{FFT}}\sum_{t=0}^{N_{FFT}-1}y_l^{ssb}(t)e^{-j\frac{2\pi}{N_{FFT}}t}
\end{equation}
\noindent in which $Y_{l,k}^{ssb}$ demonstrated the Fourier transform of the received signal in $l$th OFDM symbol and $k$th subcarrier data point.
In the next step, the SS block is extracted from the frequency domain signal. There are $N_{nre}=113$ numbers of resource elements in the SS block which are set to zero as shown in Fig. \ref{fig:ssb}. These resource elements include the information of the noise and jamming signal. The energy of these resource elements are calculated as expressed in Eq.\ref{eq:energy}.
\begin{equation}\label{eq:energy}
\begin{split}
    E &= \frac{1}{N_{nre}}\sum_{n=0}^{N_{nre}-1}{\mathcal(Y_{l,k}^{ssb}\big |_{l=0})^2}\\
    k&\in{\{0,55\}}\cup{\{184,240\}}
\end{split}
\end{equation}
The energy of noise and jammer are small in some observations. Thus, to magnify the value of energy a log function is applied to the final energy value shown in Eq.\ref{eq:log}.
\begin{equation}\label{eq:log}
    \varepsilon = \log_2(E)
\end{equation}

In the case when no jammer is present, the UE is only effected by the environmental noise. The energy of this type of interference in significantly small compared to the energy from a jammer. Thus, when the $\varepsilon$ reaches a specific threshold, it can be concluded that there is a jammer present in the scenario.

% ___________DNN Model___________ 
% DNN model structure
%% optimization problem
%% hyper parameter set table (minibatch,...)
\subsection{DL Block}
\subsubsection{DNN Input}
Observartions are designed as a 2-D image including the PSS correlation signals ($\boldsymbol{R_{pci}}, pci\in\{0,1,2\}$), and energy per null resource elements ($\varepsilon$).
In each observation ($N_{obs}\in\{1,2,...,2\mu_j\}$), first three rows in the 2-D image include correlated signal, and the last two rows are dedicated to the energy parameter (Fig. \ref{fig:block diagram}). The calculated EPNRE is one single value while the size of the correlated signal is equal to $2N_{FFT}$. Thus, to maintain the impact of the energy feature, the energy is repeated in the last two rows by being multiplied in an all-ones matrix (Eq.\ref{eq:repeat E}).

\begin{equation}\label{eq:repeat E}
    \begin{split}
        \boldsymbol{\mathcal{E}} &= \varepsilon\times{\mathbb{I}}\\
        \mathbb{I}&\in\mathbb{R}^{1\times2N_{FFT}-1}
    \end{split}
\end{equation}

After creating 2-D image of features, each observation is positioned behind the previous observation thus creating a 3-D tensor (Fig. \ref{fig:block diagram}) as the final dataset ($\boldsymbol{\chi}$).

\begin{equation}\label{eq:final dataset}
    \boldsymbol{\chi}=[\boldsymbol{\mathcal{R}}_0^T(app),\boldsymbol{\mathcal{R}}_1^T(app),\boldsymbol{\mathcal{R}}_2^T(app),\boldsymbol{\mathcal{E}}^T,\boldsymbol{\mathcal{E}}^T]^T
\end{equation}

\subsubsection{Data Augmentation and Class Balancing}
During the data generation, a noticeable dissimilarity in sample sizes between the two classes has been observed. These imbalanced classes can results in biased models and fail to generalize to minority class \cite{johnson2019survey}. This situation causes the CNN model to demonstrate less efficiency and accuracy in classifying the minority observations and decreases the performance of the model in detecting underrepresented received signals. Various techniques, including oversampling the training samples to produce a comparatively balanced dataset \cite{lv2021enhanced}, have been suggested as solutions to this problem. Additionally, research has demonstrated that CNN decisions are more difficult to generalize to minority classes when the data is unbalanced \cite{dablain2023understanding}. However, methods including data augmentation have demonstrated efficacy in enhancing the precision of classification tasks involving unbalanced datasets \cite{rojhani2023model}. To overcome the effect of the imbalance classes and use a more robust dataset, circular shift is applied to the minor dataset \cite{zhang2020circular}. Through circular shift augmentation method, each observation in the minority class is divided into sub-sequences with similar lengths, and each sub-sequence is independently shuffled to create a new sequence which introduces new variations of the collected observations. This technique, enhances the generalization capabilities of the DNN model by introducing diverse patterns.

\subsubsection{DNN Structure}
The deep learning model used for training is a supervised model, and dataset is paired with the correspondent labels as $(\boldsymbol{\chi}, \boldsymbol{\mathcal{Z}})=\{(\boldsymbol{\chi}^1,\boldsymbol{\mathcal{Z}}^1),(\boldsymbol{\chi}^2,\boldsymbol{\mathcal{Z}}^2),...,(\boldsymbol{\chi}^{\eta},\boldsymbol{\mathcal{Z}}^{\eta})\}$, where $\eta$ is the total number of observations. In this algorithm two classes are represented for the dataset, therefore, $\boldsymbol{\mathcal{Z}}^{\eta}$ represents a binary digit set and can be written using one-hot encoding (Eq.\ref{eq: label set}).
\begin{equation}\label{eq: label set}
    \boldsymbol{\mathcal{Z}}^{\eta}=\begin{cases}
        [0\ \ 1]^T\ \ \ \ for\ H_0\\
        [1\ \ 0]^T\ \ \ \ for\ H_1
    \end{cases}
\end{equation}
After normalizing using the softmax layer, the output score of the model for $\eta$th observation is expressed as follows:
\begin{equation}\label{eq: normalized z}
    \boldsymbol{O}^{\eta}=\begin{cases}
        \zeta_{H_0}(\chi^\eta|\theta)\ \ \ \ for\ H_0\\
        \zeta_{H_1}(\chi^\eta|\theta)\ \ \ \ for\ H_1
    \end{cases}
\end{equation}
\noindent where $\theta$ represents the parameter of the deep learning model, and $\zeta_{H_{0\vee1}}(\chi^\eta|\theta)\triangleq P_r\big(\chi^\eta|H_{0\vee1},\theta\big)$ denotes the jamming scores of the jamming detection problem which satisfies $\zeta_{H_{0}}(\chi^\eta|\theta)+\zeta_{H_{1}}(\chi^\eta|\theta)=1$. Based on the decision rule, two scores are compared and the output will be the hypothesis with highest score Eq. \ref{eq: decision}. 
\begin{equation}\label{eq: decision}
    \zeta_{H_{0}}(\chi^\eta|\theta)\underset{H_1}{\overset{H_0}{\gtrless}}\zeta_{H_{1\vee1}}(\chi^\eta|\theta)
\end{equation}

As the features are organized in 2-D images, the deep learning model is designed using 2-D CNN layers. Fig. \ref{fig:dnn} demonstrates the structure of the DNN model. The 3-D tensors including the features of each observation is used as an input to three layers of 2-D CNN with ReLu activation. After each layer of CNN, a batch normalization layer is added to provide a faster and more stable training. Two fully connected layers and a softmax layer is used as the last layers of the design. The softmax layer enable normalization for the output scores. A detailed list of parameters for the DNN model is provided in Table \ref{tab:hyperparameter}.

\begin{table}[htbp]
\caption{Hyperparameter Set Table}
\begin{center}
\begin{tabular}{|c|c|}
\hline
Parameter & Value \\
\hline\hline
Mini-Batch Size & 25\\
Initial Learning Rate & 0.001\\
MaxEpoch & 20\\
Validation frequency & 80\\
CNN-1 & $(2\times5) @ 256$\\
CNN-2 & $(2\times5) @ 128$\\
CNN-3 & $(1\times2) @ 128$\\
FC-1 Output Layer & 128\\
FC-2 Output Layer & 2\\
Training Optimization Method & SGDM\\
Validation Training Rate & 30\% \\
[1ex]
\hline
\end{tabular}  
\end{center}
\label{tab:hyperparameter}
\end{table}

\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=8cm, height=8cm]{figures/dnn-model.png}
    \caption{DNN model.} 
    \label{fig:dnn}
    %\vspace{-2mm}
 \end{figure}

\subsubsection{Offline Training}
% Math explanation
In the classification layer, the main goal is to maximize the probability of detection. Thus, maximizing $\zeta_{H_{0}}(\chi^\eta|\theta)$ in the absent of jammer and $\zeta_{H_{1}}(\chi^\eta|\theta)$ in the presence of jammer. To optimize the solution, and objective function can be defined as the Maximum Likelihood (ML) function represented in Eq. \ref{eq: ML}.

\begin{equation}\label{eq: ML}
    L(\theta)= \prod_{\eta=1}^{N_{obs}} \big(\zeta_{H_{0}}(\chi^\eta|\theta)\big)^{\boldsymbol{\mathcal{Z}}^{\eta}}\big(\zeta_{H_{0}}(\chi^\eta|\theta)\big)^{1-\boldsymbol{\mathcal{Z}}^{\eta}}
\end{equation}

To minimize the loss between the actual and predicted value, a negative log likelihood function is minimized to adjust the weights during the training as shown below:
\begin{equation}
\begin{split}
    \mathcal{H}(\theta)&=-\frac{1}{N_{obs}}\log(l(\theta))\\
    &=-\frac{1}{N_{obs}}\sum_{\eta=1}^{N_{obs}} \boldsymbol{\mathcal{Z}}^{\eta} \log\big(\zeta_{H_{0}}(\chi^\eta|\theta)\big)+\\
    &\ \ \ \ \  \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \ \ \  \ \ \ (1-\boldsymbol{\mathcal{Z}}^{\eta})\log\big(\zeta_{H_{1}}(\chi^\eta|\theta)\big)
\end{split}
\end{equation}
Therefore, the optimization problem can be expressed as Eq. \ref{eq: optimization dnn1}. 
\begin{equation}\label{eq: optimization dnn1}
    \Theta = \arg\min_{\theta}\mathcal{H}(\theta)
\end{equation}
Through stochastic gradient descent (SGD) optimization, the model is trained to provide higher values for $\zeta_{H_{0}}(\chi^\eta|\Theta)$ when $\boldsymbol{\mathcal{Z}}^{\eta}=[1\ \ 0]^T$ or $\zeta_{H_{1}}(\chi^\eta|\Theta)$ when $\boldsymbol{\mathcal{Z}}^{\eta}=[0\ \ 1]^T$. The training is formed through iterative back-propagating processes.


% ___________Double Threshold___________
\subsection{Accuracy Enhancement}
% histogram
% double threshold model \gamma_1, \gamma_2 (D)
\subsubsection{Double Threshold DNN}
To increase the performance of the detection algorithm, a trade-off between the $P_D$ and $P_{FA}$ should be considered. To this aim, the ratio between the two output scores can be defined as $\Gamma(\chi^\eta)=\frac{\zeta_{H_1}(\chi^\eta|\Theta)}{\zeta_{H_0}(\chi^\eta|\Theta)}$. This value is compare with a threshold to enable the algorithm to make a detection decision. However, for the scenarios when SJNR value is high, meaning that the jamming signal is weaker compared to the transmitted signal from gNB, the uncertainty is high for the classifier. Thus, the divergence between two scores $\big | \zeta_{H_0}(\chi^\eta|\Theta) - \zeta_{H_1}(\chi^\eta|\Theta)\big |$ is high and their values are too close to each other that it makes it challenging for the classifier to make a decision. In other words, defining one hard decision threshold of 0.5 reduces the accuracy of the jamming detector in the uncertainty area. Therefore, an ambiguity area is defined to reach a better and more accurate decision. Based on this, while the decision is being made out of the ambiguity area, the detector detects the absence or the presence of the jammer with 100\% empirical accuracy. To design such structure, two threshold points ($\gamma^{(1)}_1=\Gamma\big(\boldsymbol{\chi}_s^{\eta_1^*}\big), \gamma^{(1)}_2=\Gamma\big(\boldsymbol{\chi}_s^{\eta_2^*}\big)$) are considered. $\boldsymbol{\chi}_s$ represents sorted observations in a descending fashion, and $\eta_1^*, \eta_2^*$ are observations which fall in the areas that the classification decides with high certainty and is defined in Eq. \ref{eq: eta1} and Eq. \ref{eq: eta2}.
\begin{numcases}{}\label{eq: eta1}
        \eta^*_1=\arg\min_{\eta}\big(\zeta^{(1)}_{H_0}(\boldsymbol{\chi}_s^\eta|\Theta)<\zeta^{(1)}_{H_1}(\boldsymbol{\chi}_s^\eta|\Theta)\big)\\
        \label{eq: eta2}
        \eta ^*_2=\arg\max_{\eta}\big(\zeta^{(1)}_{H_0}(\boldsymbol{\chi}_s^\eta|\Theta)>\zeta^{(1)}_{H_1}(\boldsymbol{\chi}_s^\eta|\Theta)\big)
\end{numcases}
While $\Gamma(\chi^\eta)>\gamma^{(1)}_1$ or $\Gamma(\chi^\eta)<\gamma^{(1)}_2$, the detector selects $H_0$ or $H_1$ respectively. In the case that $\gamma^{(1)}_2<\Gamma(\chi^\eta)<\gamma^{(1)}_1$, another DNN is trained specifically for higher SJNR values is activated and observation are fed for more accurate analysis to this DNN. This improves the performance of the jamming detection by  minimizing the probability of miss-detection and false-alarm. The structure of the double threshold DNN model is represented in Algorithm 1. After data is processed in the data preprocessing block, it is fed into the first DNN with double threshold design. The first DNN calculates $\zeta^{(1)}_{H_0}(\boldsymbol{\chi}_s^\eta|\Theta)$ and $\zeta^{(1)}_{H_1}(\boldsymbol{\chi}_s^\eta|\Theta)$ which are the weight scores correspondence to this block. These scores are then used as input to the first threshold and decision block. If the scores represent values outside of the uncertainty area, the final decision $Q_1$ is provided as an output. In the case that the score values are fallen into the uncertainty area, data is sent to the second DNN with single threshold design for final classification. The second DNN is trained based on more fine features, thus, has more accuracy compared to the first DNN. In the second DNN, the threshold $\gamma^{(2)}$ is used to detect the jammer in harsher conditions (higher SJNR values). The ratio between the two output scores of the second DNN, $\zeta^{(2)}_{H_1}(\hat{\chi})$ and $\zeta^{(2)}_{H_0}(\hat{\chi})$, is defined as $\Gamma^{(2)}(\chi^\eta)=\frac{\zeta^{(2)}_{H_1}(\hat{\chi})}{\zeta^{(2)}_{H_0}(\hat{\chi})}$. The comparison between the ratio $\Gamma^{(2)}(\chi^\eta)$ and detection threshold $\gamma^{(2)}$ enables a degree of freedom to have a trade-off between $P_D$ and $P_{FA}$. After finding the $\Gamma^{(2)}(\chi^\eta)$ using optimum parameters of $\Theta$ and the $H_0$, empirical $P_{FA}$ can be computed to determine the threshold value. Assume we define the target value for $P_{FA}$ as $\delta_{FA}$ so that $P_{FA} \leq \delta_{FA}$, and we define total number of observations fallen into $H_0$ hypothesis as $N_{H_0}$. After sorting the observations in a descending order ($\chi_s^\eta$), the $\gamma^{(2)}$ threshold can be defined as Eq. \ref{eq: gamma2}. 
\begin{equation}\label{eq: gamma2}
    \gamma^{(2)}=\Gamma^{(2)}\big(\chi_s^\eta \lfloor \delta_{FA} N_{H_0} \rfloor;\Theta \big)
\end{equation}
The classification is processed based on comparing the scores ratio and single threshold value in the second dNN. 
During the online detection, samples are used as input to the DNN block and after evaluations and passing through the softmax layer, two output scores are presented. The final decision is made in threshold and decision block using $\gamma^{(2)}$ as below:
\begin{equation}
    \Gamma^{(2)}(\chi_{online})\underset{H_1}{\overset{H_0}{\gtrless}}\gamma^{(2)}
\end{equation}
\noindent in which $\chi_{online}$ represents the online samples. Fig. \ref{fig:dnn2} provides an overall overview of the structure of the double threshold enabled design explained above.

% optimization problem (-10 to 20 dB)

\begin{comment}
\begin{numcases}{}\label{eq: gamma1}
    \gamma^{(1)}_1=\Gamma\big(\boldsymbol{\chi}_s^{\eta_1^*}\big)\\
    \label{eq: gamma2}
    \gamma^{(1)}_2=\Gamma\big(\boldsymbol{\chi}_s^{\eta_2^*}\big)
\end{numcases}
\end{comment}

%\end{comment}


\begin{comment}
\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=8.5cm, height=2.5cm]{figures/dnn2.png}
    \caption{Adding another DNN block to improve the accuracy.} 
    \label{fig:dnn2}
    %\vspace{-2mm}
 \end{figure}

\begin{algorithm}
\caption{Double Threshold DNN - Online Detection}\label{alg:cap}
\begin{algorithmic}[1]
\State Set $\hat{\chi}$ as the current observation
\State Set $\gamma^{(1)}_1=\Gamma\big(\hat{\chi}), \gamma^{(1)}_2=\Gamma\big(\hat{\chi})$
\State Calculate $\zeta^{(1)}_{H_0}(\hat{\chi}), \zeta^{(1)}_{H_1}(\hat{\chi})$
\State Calculate $\Gamma^{(1)}=\frac{\zeta^{(1)}_{H_1}(\hat{\chi})}{\zeta^{(1)}_{H_0}(\hat{\chi})}$

\If{$\Gamma^{(1)}>\gamma^{(1)}_1$}
    \State The classification decides $H_0$
\ElsIf{$\Gamma^{(1)}<\gamma^{(1)}_2$}
    \State The classification decides $H_1$
\ElsIf{$\gamma^{(1)}_2<\Gamma^{(1)}<\gamma^{(1)}_1$}
    \State Activate DNN-2
    \State Calculate $\zeta^{(2)}_{H_0}(\hat{\chi}), \zeta^{(2)}_{H_1}(\hat{\chi})$
    \State Calculate $\Gamma^{(2)}=\frac{\zeta^{(2)}_{H_1}(\hat{\chi})}{\zeta^{(2)}_{H_0}(\hat{\chi})}$
    \If{$\Gamma^{(2)}>\gamma^{(2)}$}
      \State The classification decides $H_0$
    \ElsIf{$\Gamma^{(2)}<\gamma^{(2)}$} 
      \State The classification decides $H_1$
    \EndIf  
\EndIf
%\EndWhile
\end{algorithmic}
\end{algorithm}


 \subsubsection{Deep Cascade Learning}
 % to avoid vanishin gradient problem due to low dynamic range of SJNR in our dataset
 %% it accommodates the nonlinear relationship between input and output by not eliminating the linear relationship between the two
 %% efficient training of deep neural networks in a bottom-up fashion using a layered
 %% when sjnr values are close to each other and classifier has troubles classify between two classes so it fine tunes the weights
 Although the convolution network has demonstrated remarkable performance and results, it experiences the vanishing gradient problem while undergoing training. This occurs because the weight updates are substantially reduced for initial layers due to low dynamic range of SJNR in our dataset. One solution to overcome this situation is deep cascade learning algorithm proposed in \cite{marquez2018deep}. Deep cascade learning gradually trains the network from the lowest to higher layers. When jamming signal is weak and SJNR values are close together, the classifier faces troubles classify between two classes. Deep cascade learning fine-tunes the weights by dividing the network to sub-layers and sequentially trains each layer until all the input layers have been trained. Through this technique, the vanishing gradient problem can be eliminated by compelling each layer of the network to acquire features that are correlated with the output. In other words, it maintains the linear correlation between input and output while accommodating the nonlinear relationship. Furthermore, it has shown reduction of training time and memory while adjusting the complexity of the network to the given data. The structure of the DNN model using deep cascade learning is shown in Fig. \ref{fig: dcl}. The input layer in connected to the output using two dense layers. The weights for the initial model layer and the output are subsequently obtained via back-propagation algorithm during the training. After reaching a state of stability, the second layer is trained by connecting to an output layer with similar structure to the first layer using data created by forward propagating the actual inputs through the fixed initial layer. Through several iterations, every layer goes through this process to be learned, and the weights remain constant for the subsequent layer. Adapting this approach helps to increase robustness of the second DNN and preserve the back-propagated gradient while having hidden layers. 
\graphicspath{{figures/}}
%\vspace{-5mm}
\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figures/cascade.png}
    \caption{Deep Cascade Learning} 
    \label{fig: dcl}
    %\vspace{-2mm}
 \end{figure}

\end{comment}
